Federated Learning from Only Unlabeled Data with Class-Conditional-Sharing Clients

Supervised federated learning (FL) enables multiple clients to share the trained model without sharing their labeled data. However, potential clients might even be reluctant to label their own data, which could limit the applicability of FL in practice. In this paper, we show the possibility of unsupervised FL whose model is still a classifier for predicting class labels, if the class-prior probabilities are shifted while the class-conditional distributions are shared among the unlabeled data owned by the clients. We propose federation of unsupervised learning (FedUL), where the unlabeled data are transformed into surrogate labeled data for each of the clients, a modified model is trained by supervised FL, and the wanted model is recovered from the modified model. FedUL is a very general solution to unsupervised FL: it is compatible with many supervised FL methods, and the recovery of the wanted model can be theoretically guaranteed as if the data have been labeled. Experiments on benchmark and real-world datasets demonstrate the effectiveness of FedUL. Code is available at https://github.com/lunanbit/FedUL.

==> Federated Learning with Only Unlabeled Datasets final/cmds.tex <==
\makeatletter
% Taken from http://ctan.org/pkg/centernot
\newcommand*{\centernot}{%
  \mathpalette\@centernot
}
\def\@centernot#1#2{%
  \mathrel{%
    \rlap{%
      \settowidth\dimen@{$\m@th#1{#2}$}%
      \kern.5\dimen@
      \settowidth\dimen@{$\m@th#1=$}%
      \kern-.5\dimen@
      $\m@th#1\not$%
    }%
    {#2}%
  }%
}
\makeatother
\newcommand{\independent}{\perp\mkern-9.5mu\perp}
\newcommand{\dependent}{\centernot{\independent}}



% \newtheorem{theorem}{Theorem}[section]
\newtheorem{rul}[theorem]{Rule}

==> Federated Learning with Only Unlabeled Datasets final/related.tex <==
\section{Related Works}

To the best of our knowledge, this is the first work addressing the FL with only unlabeled datasets

\paragraph{Federated learning}
Federated learning is an emerging paradigm in distributed machine learning, which allows different clients collaboratively train model together without data sharing. One of the most popular FL paradigm is called FedAvg~\cite{mcmahan2017communication}. FedAvg is a easy-to-implement distributed learning strategy by aggregating local model updates on the server side and transmitting the averaged model back to local clients. For IID data, FL has been proven effective. However, in practice, data mostly distribute as non-IID. Non-IID data could substantially degrade the performance of FL models~\cite{zhao2018federated,li2019convergence, li2021fedbn}. Several approaches have been proposed to address the non-IID issue. FedProx \citep{li2018federated}, a recent provable framework tackled the heterogeneity by adding a proximal term to FedAvg to regularize local model weights updates. Scaffold~\cite{karimireddy2020scaffold} corrects the local updates by variance reduction. FedRobust \citep{reisizadeh2020robust} assumes data follows an affine distribution shift and tackles this problem by learning the affine transformation. FedBN~\cite{li2021fedbn} keeps all BN parameters strictly local to reduce the effect of feature shift. However, almost all of theses existing FL studies demonstrate that their approaches are better than FedAvg on  non-IID data in supervised learning only. It is still an open question whether FedAvg is a feasible strategy for unlabeled data leanring. 

% Add Personalized non-IID

% Add Weakly Supervsied FL



%Introduce standard FedAvg, non i.i.d.

\paragraph{Unlabeled data learning}

\begin{itemize}
    \item Federated Learning with Only Positive Labels (ICML2020) \url{http://www.sanjivk.com/FedPositive_ICML20.pdf};
    \item Federated Semi-Supervised Learning with Inter-Client Consistency and Disjoint Learning (ICLR2021) \url{https://arxiv.org/pdf/2006.12097.pdf}
    \item FEDAUX: Leveraging Unlabeled Auxiliary Data in Federated Learning (arxiv) \url{https://arxiv.org/pdf/2102.02514.pdf};
    \item Federated Learning with Positive and Unlabeled Data (arxiv) \url{https://arxiv.org/pdf/2106.10904v1.pdf};
    \item SemiFL: Communication Efficient Semi-Supervised Federated Learning with Unlabeled Clients (arxiv) \url{https://arxiv.org/pdf/2106.01432.pdf}.
    \item Learning from Corrupted Binary Labels via Class-Probability Estimation, ICML2015,
    \url{http://proceedings.mlr.press/v37/menon15.pdf}
    \item Learning from Label Proportions with Generative Adversarial Networks, NIPS2019
    \url{https://arxiv.org/abs/1909.02180}
    \item On the minimal supervision for training any binary classifier from only unlabeled data, ICLR2019, 
    \url{https://arxiv.org/abs/1808.10585}
    \item Mitigating overfitting in supervised classification from two unlabeled datasets: A consistent risk correction approach, AISTATS2020, \url{https://arxiv.org/abs/1910.08974}
    \item Learning from label proportions: A mutual contamination framework, NIPS2020, \url{https://arxiv.org/abs/2006.07330}
    \item Learning from label proportions with consistency regularization, ACML2020,  \url{https://www.csie.ntu.edu.tw/~htlin/paper/doc/acml20llpvat.pdf}
\end{itemize}




==> Federated Learning with Only Unlabeled Datasets final/sections/app_notation.tex <==

\setcounter{table}{0}
\setcounter{figure}{0}
% \renewcommand{\thetable}{A\arabic{table}}
\renewcommand\thetable{\thesection.\arabic{table}}
\renewcommand\thefigure{\thesection.\arabic{figure}}    


% \section{Data and Code Availability}
% \label{app:code}
% The trained models, guidelines for data downloading and preparation, code for training, validation, testing of all the methods, readme file, libraries requirement, and environment setup for our benchmark experiments are available at the \textbf{anonymous link}: \href{https://drive.google.com/drive/folders/1kcMO0_XoxoPFhv1ZgcZ6bV_HTzZo-zPs?usp=sharing}{https://drive.google.com/drive/folders/1kcMO0\_XoxoPFhv1ZgcZ6bV\_HTzZo-zPs?usp=sharing}. Due to size limitation, we could not share the preprocessed large scale real-world datasets. We are very happy to release all materials in the final version.


\section{Notation Table}
\label{app:notation_table}
\begin{table}[ht]
\caption{Notations used in the paper.}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cl}
\hline
Notations & Description \\ \hline \\[-1.8ex]
$d$ & input dimension \\[0.1ex]
$K$ & number of classes for the original classification task \\[0.1ex]
$k$ & index of the class $k\in[K]$ \\[0.1ex]
$\mathcal{X}$ & input space $\mathcal{X}\subset\R^d$ \\[0.1ex] 
$\mathcal{Y}$ & label space $\mathcal{Y}=[K]$ where $[K]\coloneqq\{1,\ldots,K\}$ \\[0.1ex] 
$\bx$ & input $\bx \in \mathcal{X}$ \\[0.1ex]
$y$ & true label $y \in \mathcal{Y}$ \\[0.1ex]
$p$ & test data distribution \\[0.1ex]
$\pi^k$ & $k$-th class prior $\pi^k\coloneqq p(y=k)$ of the test set \\[0.1ex]
$\bpi$ & vector form of $\pi^k$ where $\bpi=[\pi^1,\cdots,\pi^K]^\top$ \\[0.1ex]
% $\D_S$ & joint distribution over all seen clients \\[0.1ex]
$\ell$ & loss function for a classification task \\[0.1ex]
$R$ & risk for the original FL task \\[0.1ex]
$\boldf$ & global model predicting label $y$ for input $\bx$ \\[0.1ex]
$C$ & number of clients in the FL setup \\[0.1ex]
$c$ & index of the client $c\in[C]$ \\[0.1ex]
$\fc$ & $c$-th client model predicting label $y$ for input $\bx$ \\[0.1ex]
% $\D$ & the joint distribution over all seen and unseen clients \\ [0.1ex]
$p_c$ & local data distribution at the $c$-th client \\[0.1ex]
$n_c$ & number of training data at the $c$-th client \\[0.1ex]
$\mathcal{D}_c$ & labeled training set $\mathcal{D}_c = \{(\bx^c_i,y^c_i)\}_{i=1}^{n_c}$ at the $c$-th client \\[0.1ex]
% $n_c$ & size of samples drawn from distribution for the $c$-th client \\[0.1ex]
$\alpha_l$ & local step size \\[0.1ex]
$\alpha_g$ & global step size \\[0.1ex]
$R$ & global communication round \\[0.1ex]
$L$ & local updating iterations \\[0.1ex]
$M_c$ & number of available U sets at the $c$-th client \\[0.1ex]
$m$ & index of the U set $m\in[M_c]$ \\[0.1ex]
$n_{c,m}$ & number of training data in the $m$-th U set at the $c$-th client \\[0.1ex]
$p_c^{m}$ & $m$-th U data distribution at the $c$-th client \\[0.1ex] 
$\mathcal{U}_{c}^m$& $m$-th U set at the $c$-th client $\mathcal{U}_{c}^{m} = \{\bx_{i}^{c,m}\}_{i=1}^{n_{c,m}}$ \\[0.1ex]
$\mathcal{U}_{c}$ &  all available U sets at the $c$-th client $\mathcal{U}_{c}=\{\mathcal{U}_{c}^{m}\}_{m=1}^{\mc}$ \\[0.1ex]
$M$ & the maximum number of available U sets among all clients $M=\max_{c\in[C]}M_c$ \\[0.1ex]
$\pi_{c}^{m,k}$ & $k$-th class prior $\pi_{c}^{m,k}=p_{c}^{m}(y = k)$ of the $m$-th U set at the $c$-th client \\[0.1ex]
$\Pi_c$ & matrix form of $\pi_{c}^{m,k}$ where $\Pi_c\in\R^{\mc\times K}$ \\[0.1ex]
$\overline{y}$ & surrogate label $\bar{y} \in [M]$ \\[0.1ex]
$\overline{p}_c$ & surrogate local data distribution at the $c$-th client \\[0.1ex]
$\overline{\mathcal{U}}_{c}$ & surrogate labeled training set $\overline{\mathcal{U}}_{c}=\{\bx_i,\overline{y}_i\}_{i=1}^{n_c}$ at the $c$-th client \\[0.1ex]
$\overline{\pi}^m_c$ & $m$-th surrogate class prior $\overline{\pi}^m_c=\overline{p}_c(\overline{y}=m)$ at the $c$-th client \\[0.1ex]
$\overline{\bpi}_c$ & vector form of $\overline{\pi}^m_c$ where $\overline{\bpi}_c=[\overline{\pi}^1_c,\cdots,\overline{\pi}^{M}_c]^\top$ \\[0.1ex]
$\bg$ & surrogate global model predicting surrogate label $\overline{y}$ for input $\bx$ \\[0.1ex]
$\overline{\boldeta}_c$ & surrogate class-posterior probability at the $c$-th client where $(\overline{\boldeta}_c(\bx))_m=\overline{p}_c(\overline{y}=m\mid\bx)$ \\[0.1ex]
$\boldeta$ & true class-posterior probability at the $c$-th client where $(\boldeta(\bx))_k=p(y=k\mid\bx)$ \\[0.1ex]
$\bQ_c$ & vector-valued transition function $\bQ_c: (\mathcal{X}\to\Delta_K)\to(\mathcal{X}\to\Delta_{M})$ \\[0.1ex]
$J$ & surrogate risk for the surrogate FL task \\[0.1ex]
\hline
\end{tabular}%
}
\label{tab:notation}
\end{table}


==> Federated Learning with Only Unlabeled Datasets final/sections/app_related.tex <==
\newpage
\section{Related Work}
\label{sec:related}%
\subsection{Personalized Federated Learning}
Considering the heterogeneity of data, clients, and systems, personalization is a natural and trending solution to improve FL performance. 
Many efforts have been made in personalized FL.
% to address the challenges of heterogeneity.
FedProx\citep{li2018federated}, FedCurv~\citep{shoham2019overcoming}, and FedCL~\citep{yao2020continual} propose regularization-based methods that include special regularization terms to improve FL model generalizing to various clients.
Meta-learning methods, such as MAML~\citep{finn2017model}, are also used to learn personalized models for each client
% train highly adaptable models to achieve personalization
\citep{jiang2019improving,fallah2020personalized,li2019differentially}.
% Another view of the personalized FL is to see it as a multi-task learning problem where
Unlike the methods mentioned above that yield a single generalizable model, 
multiple FL models can be trained using clustering strategies \citep{sattler2020clustered,ghosh2020efficient}.
Different local FL models can also be achieved by changing the last personalized layers~\citep{li2021fedbn,arivazhagan2019federated}.

At first glance, FedUL looks similar to personalized FL since each client learns a "personalized" model $\bg_c$ which contains a client-specific transition layer $\bQ_c$. However, our learning setting and method are very different from existing personalized FL approaches, as explained below.
First, our framework focuses on FL with only unlabeled data.
The personalized model $\bg_c$ only serves as a proxy, in order to be compatible with the transformed unlabeled data, and our ultimate goal is to learn $\boldf$ that is not exactly personalized. 
Specifically, 1) if the inter-clients are IID, FedUL yields the same proxy model $\bg_c$ and federated model $\boldf$ for all the clients; 2) if the inter-clients are Non-IID, although $\bg_c$ is different (as $\bQ_c$ is different), the underlying model $\boldf$ (what we want) is still the same.
Second, our method differs from the previous personalized FL methods by its surrogate training nature: it works as a wrapper that transforms unlabeled clients to (surrogate) labeled ones and is compatible with many supervised FL methods.

\subsection{Semi-supervised Federated Learning}
Another line of research working on utilizing unlabeled data in FL follows the semi-supervised learning framework \citep{zhu2005semi,chapelle06SSL}, which assumes a small amount of labeled data available at the client side (labels-at-client) or at the server side (labels-at-server).
% FedSem employs pseudo-labeling technique to generate fake labels for unlabeled data based on the trained FedAvg model with labeled data. 
% The data with pseudo labels are further used to retrain FedAvg to obtain the final global model. 
% Thus, FedSem easily overfits to imperfect annotations from the pre-trained FedAvg and further leads to unsatisfactory performance. 
For example,
FedMatch \citep{jeong2020federated} introduces a new inter-client consistency loss that maximizes the agreement between multiple clients and decomposes the model parameters into one for labeled data and the other for unlabeled data for disjoint learning.
FedSem \citep{albaseer2020exploiting} generates pseudo labels for unlabeled data based on the trained FedAvg model with labeled data, and the generated (pseudo) labeled data are further used to retrain FedAvg to obtain the global model.
Moreover, distillation-based semi-supervised FL \citep{itahara2020distillation} considers using shared unlabeled data for distillation-based message exchanging.
% trains and aggregates the model parameters of the labeled server and unlabeled clients in parallel.

Although the motivation of FedUL can be related to semi-supervised FL since both work on utilizing unlabeled data in FL, our learning setting is different since we only have unlabeled data at both the client and the server sides, and our method is different since FedUL follows the empirical risk minimization framework.



==> Federated Learning with Only Unlabeled Datasets final/sections/app_roadmap.tex <==
\paragraph{Roadmap} The appendix is organized as follows. 
% We point to the shareable code and preprocessed data in Section~\ref{app:code} . 
We summarize notations used in our paper in Section~\ref{app:notation_table} and give a full discussion of related work in Section~\ref{sec:related}.
Our proofs are presented in Section~\ref{sec:proof}. 
We provide detailed experimental settings in Section~\ref{app:exp} and supplementary experimental results on the benchmark datasets in Section~\ref{app:more}.

==> Federated Learning with Only Unlabeled Datasets final/sections/conclusion.tex <==
\section{Conclusion}
% This paper is an important initial step towards formally demonstrate the feasibility for the federated of unsupervised learning in multi-class classification tasks. 
In this paper, we propose FedUL, a novel FL algorithm using only U data. 
FedUL works as a wrapper that transforms the unlabeled client data and modifies the client model to form a surrogate supervised FL task, which can be easily solved using existing FL paradigms. 
Theoretically, we prove that the recovery of the optimal model by using the FedUL method can be guaranteed under mild conditions.
% the optimal model learned by supervised FL can be recovered from the FedUL training scheme under mild conditions.
Through extensive experiments on benchmark and real-world datasets, we show FedUL can significantly outperform the baseline methods under different settings. As a wrapper, we expect FedUL can be further improved by incorporating advanced FL aggregation or optimization schemes for the non-IID setting~\citep{wang2020tackling,li2018federated,li2021fedbn,karimireddy2020scaffold}. 
% We also plan to evaluate FedUL with larger datasets and a larger scale of clients as the future work.

==> Federated Learning with Only Unlabeled Datasets final/sections/experiment.tex <==
\section{Experiments}
% To do list: \\
% 1. Client Non-IID setting with 1 class dominate 80\% (MNIST): Clients 5 Sets (10 20 40) for FedPL, FedLLP, FedLLP-VAT, FedUU, Supervised, 10\% Supervised\\

% 1. medical dataset (four self-designed baselines, 12-24-48 single run) Expected to complete on: \textcolor{red}{Sep/21 (Tue)}  \\

% 2. Client IID setting (MNIST): Clients 5 Sets (10 20 40) for FedPL, FedLLP, FedLLP-VAT, FedUU, Supervised,\\

% 2. semi-supervised published method baseline (benchmark datasets only),we vary num of data on the server (0, 1000, 5000 labeled samples).
% \begin{itemize}
%     \item Fed Cluster (WangZhao by next weekend)
%     \item Fed Semi Inter-Client(ICLR2021) (Xiaoxiao try)
%     \item Ours (Wang Zhao by next weekend, CIFAR)
%     %\item Fed Mixup
% \end{itemize}
% 3. local update step (done) \\
% 4. training batch size (done) \\
% 5. noise ratio (done)

In this section, we conduct experiments to validate the effectiveness of the proposed FedUL method under various testing scenarios. 
Compared with the baseline methods,
% alternative strategies, 
FedUL consistently achieves superior results on both benchmark and real-world datasets. The detailed experimental settings and additional supportive results are presented in Appendix~\ref{app:exp} \&~\ref{app:more}.

\subsection{Benchmark Experiments}
\label{subsec:benchmark}
\textbf{Setup:}
As proof-of-concepts, we first perform experiments on widely adopted benchmarks MNIST \citep{lecun1998gradient} and CIFAR10 \citep{krizhevsky2009learning}. 
% For all experiments, we split 20\% data for validation and model selection.
We generate $M$ sets of U training data according to \eqref{ptr} for each client $c\in[C]$. 
The total number of training samples $\overline{n}_c$ on each client is fixed, and the number of instances contained in each set indexed by $m$ is also fixed as $\overline{n}_c/M$. 
In order to simulate the real world cases, we uniformly select class priors $\pi_{c}^{m,k}$ from range $[0.1, 0.9]$ and then regularize them to formulate a valid $\Pi_c\in\R^{M\times K}$ as discussed in Section~\ref{sec:formulate}.
% We find that the generated class priors are not all identical, 
% % \Nan{what we do is to check whether the assumption of full column rank matrix $\bpi_c\in\R^{m\times K}$ is satisfied}
% which is often the case, to make sure the problem is mathematically solvable. 
% Note that the class priors are determined before sampling and are not all equal in our setup, which is more realistic and essentially different from the uniform set generation setup used in most LLP literature. \Xiaoxiao{Do we need to highlight here. I feel the current tongue sounds like our limitation that we need such a special setting.}

For model training, we use the cross-entropy loss and Adam \citep{kingma2014adam} optimizer with a learning rate of $1e{-4}$ and train 100 rounds. If not specified, our default setting for local update epochs (E) is $1$ and batch size (B) is $128$ with $5$ clients (C) in our FL system. We use LeNet  \citep{lecun1998gradient} and ResNet18 \citep{he2016deep} as backbone for MNIST and CIFAR10, respectively.
Here, we investigate two different FL settings: {\bf IID} and {\bf Non-IID}, where the overall label distribution across clients is the same in the IID setting, whereas clients have different label distributions in the non-IID setting.
% Every client has its own data distribution in Non-IID setting, while the same data distribution in IID setting.
Specially, for Non-IID setting, we impose class-prior shift as follows:
\begin{itemize}[leftmargin=1em, itemsep=1pt, topsep=1pt, parsep=1pt]
    % \item The classes are divided into the majority and minority classes, where the fraction of the minority classes is $\mu \textless 0.08$ while the fraction of the majority classes is $\mu$ from range $[0.15, 0.25]$.
    \item the classes are divided into the majority and minority classes, where the fraction of each minority class is less than $0.08$ while the fraction of each majority class is in the range $[0.15, 0.25]$;
    \item the training data for every client are sampled from $2$ majority classes and $8$ minority classes;
    \item the test data are uniformly sampled from all classes.
\end{itemize}


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{paper/figures/mnist_ablation.pdf}
%     \caption{Ablation studies on MNIST. (a) effects of accessible clients amount on the model performance; (b) analysis of local updating epochs on the model performance; (c) how batch size influence the performance and stability of model.}
%     \label{fig:mnist_ablation}
% \end{figure}

% Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[t]
% \renewcommand\arraystretch{1.1}
% \centering
% \caption{Quantitative comparison of our method with the baseline methods on benchmark datasets under Non-IID and IID setting (mean (std)). The best method (paired t-test at significance level 5\%) is highlighted in boldface.} 
% % \Xiaoxiao{Pls add explanation for `Avg\%' :)}
% \label{tb:comp_sota}
% \scalebox{0.85}{
%     \begin{tabular}{c|c|ccc|c|c}
%     \toprule
%     \multicolumn{7}{l}{\textbf{IID Task with 10 Clients}} \\
%     \midrule
%     \midrule
%     Dataset & Sets  & FedPL & FedLLP & FedLLP-VAT & FedUL & FedAvg 10\% \\
%     \midrule
%     \multirow{3}[2]{*}{MNIST} & 10    & 2.19 (0.04) & 10.11 (7.12) & 25.83 (22.64) & \textbf{0.74 (0.14)} & \multirow{3}[2]{*}{1.58 (0.23)} \\
%           & 20    & 2.55 (0.30) & 24.23 (17.52) & 28.40 (23.20) & \textbf{1.05 (0.05)} &  \\
%           & 40    & 3.13 (0.25) & 32.53 (16.93) & 34.46 (15.46) & \textbf{1.47 (0.11)} &  \\
%     \midrule
%     \multirow{3}[2]{*}{CIFAR10} & 10    & 40.47 (0.58) & 76.23 (1.47) & 76.25 (1.65) & \textbf{20.40 (0.63)} & \multirow{3}[2]{*}{33.57 (1.03)} \\
%           & 20    & 46.44 (0.71) & 78.10 (3.58) & 76.26 (3.83) & \textbf{21.61 (0.23)} &  \\
%           & 40    & 51.58 (1.18) & 79.10 (2.34) & 80.44 (1.60) & \textbf{22.71 (0.17)} &  \\
%     \midrule
%     \multicolumn{7}{l}{\textbf{Non-IID Task with 10 Clients}} \\
%     \midrule
%     \midrule
%     Dataset & Sets  & FedPL & FedLLP & FedLLP-VAT & FedUL & FedAvg 10\% \\
%     \midrule
%     \multirow{3}[2]{*}{MNIST} & 10    & 12.24 (1.36) & 20.81 (14.72) & 17.26 (10.39) & \textbf{1.91 (0.16)} & \multirow{3}[2]{*}{3.03 (0.24)} \\
%           & 20    & 5.73 (0.89) & 17.67 (11.48) & 18.45 (4.30) & \textbf{1.45 (0.27)} &  \\
%           & 40    & 4.16 (0.56) & 14.98 (10.11) & 13.62 (5.47) & \textbf{1.27 (0.12)} &  \\
%     \midrule
%     \multirow{3}[2]{*}{CIFAR10} & 10    & 68.53 (1.14) & 84.11 (2.63) & 82.17 (2.58) & \textbf{39.20 (0.79)} & \multirow{3}[2]{*}{52.48 (1.55)} \\
%           & 20    & 61.49 (1.42) & 71.69 (7.59) & 72.34 (7.39) & \textbf{34.12 (0.57)} &  \\
%           & 40    & 55.89 (2.19) & 58.21 (4.95) & 59.42 (9.59) & \textbf{32.21 (1.02)} &  \\
%     \bottomrule
%     \end{tabular}}%
%     \vspace{-5mm}
% \end{table}%


%previous 5 clients table
\begin{table}[t]
\renewcommand\arraystretch{1.1}
\centering
\caption{Quantitative comparison of our method with the baseline methods on benchmark datasets under IID and Non-IID setting (mean error (std)). The best method (paired t-test at significance level 5\%) is highlighted in boldface.}
\vspace{1ex}
% \Xiaoxiao{Pls add explanation for `Avg\%' :)}
\label{tb:comp_sota}
\scalebox{0.88}{
% \scalebox{1}{
\begin{tabular}{c|p{1cm}<{\centering}|ccc|c|c}
\toprule
\multicolumn{7}{c}{\leftline{\textbf{IID Task with 5 Clients}}}\\
\hline\hline
Dataset&Sets&FedPL&FedLLP&FedLLP-VAT&FedUL&FedAvg 10\%\\
\hline
\multirow{3}{*}{MNIST}  & 10 & 2.12 (0.10) & 19.00 (15.90) & 20.53 (5.39) & \bf 0.78 (0.06) & \multirow{3}{*}{1.79 (0.09)} 
 \\
 & 20 & 2.98 (0.15) & 4.38 (3.95) & 4.40 (5.11) & \bf 1.12 (0.09) &\\
 & 40 & 3.90 (0.22) & 10.11 (15.74) & 11.96 (9.56) & \bf 1.00 (0.29) &\\
 \hline
\multirow{3}{*}{CIFAR10}  & 10 & 34.60 (0.30) & 77.01 (5.02) & 77.56 (8.71) & \bf 18.56 (0.04) & \multirow{3}{*}{32.85 (1.03)} 
 \\
 & 20 & 42.06 (1.63) & 78.74 (6.96) & 84.18 (5.95) & \bf 19.66 (0.30) &\\
 & 40 & 46.20 (0.67) & 73.75 (4.78) & 78.65 (6.91) & \bf 20.31 (0.69) &\\
\midrule
\multicolumn{7}{c}{\leftline{\textbf{Non-IID Task with 5 Clients}}}\\
\hline\hline
Dataset&Sets&FedPL&FedLLP&FedLLP-VAT&FedUL&FedAvg 10\%\\
\hline
\multirow{3}{*}{MNIST}  & 10 & 15.54 (3.48) & 20.52 (15.00) & 23.39 (15.34) & \bf 2.98 (1.72) & \multirow{3}{*}{3.82 (1.56)} 
 \\
& 20 & 7.54 (2.77) & 6.63 (7.94) & 11.76 (6.60) & \bf 1.77 (0.49)
 \\
 & 40 & 5.76 (0.90) & 5.53 (2.51) & 7.82 (10.73) & \bf 1.64 (0.18)
 \\\hline
 \multirow{3}{*}{CIFAR10} & 10 & 70.65 (2.38) & 81.12 (5.41) & 81.55 (7.09) & \bf 42.92 (3.02) &
 \multirow{3}{*}{58.62 (8.63)} 
 \\
& 20 & 63.53 (1.24) & 65.51 (13.16) & 70.51 (7.66) & \bf 35.24 (0.98)
 \\
& 40 & 53.78 (0.13) & 65.72 (3.93) & 60.23 (5.71) & \bf 31.43 (1.72)
 \\
\bottomrule
\end{tabular}
}
\vspace{-5mm}
\end{table}
% previous 5 clients table end


%\fi

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\iffalse
\begin{table}[t]
\renewcommand\arraystretch{1.1}
\centering
\caption{Quantitative comparison of our method with the baseline methods on benchmark datasets under IID and Non-IID setting (mean error (std)). The best method (paired t-test at significance level 5\%) is highlighted in boldface.}
\label{tb:comp_sota}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|cccc|c|cccc|c}
\midrule
 &  & \multicolumn{5}{c|}{\bf IID Task with Five Clients} & \multicolumn{5}{c}{\bf Non-IID Task with Five Clients} \\ \hline \hline
\multicolumn{1}{c|}{Dataset} & Sets & FedPL & FedLLP & \begin{tabular}[c]{@{}c@{}}FedLLP\\ -VAT\end{tabular} & \begin{tabular}[c]{@{}c@{}}\bf FedUL \\ \bf (ours) \end{tabular}  & \begin{tabular}[c]{@{}c@{}}FedAvg\\ 10\% \end{tabular} & FedPL & FedLLP & \begin{tabular}[c]{@{}c@{}}FedLLP\\ -VAT\end{tabular} & \begin{tabular}[c]{@{}c@{}}\bf FedUL \\ \bf(ours) \end{tabular} & \begin{tabular}[c]{@{}c@{}}FedAvg\\ 10\% \end{tabular}\\ \hline
\multicolumn{1}{c|}
{\multirow{6}{*}{MNIST}} & \multirow{2}{*}{10} & 2.12 & 19.00 & 20.53 & \bf 0.78 & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}1.79\\ (0.09)\end{tabular}} & 15.54 & 20.52 & 23.29 & \bf 2.98 & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}3.82\\ (1.56)\end{tabular}} \\ %\cline{3-6} \cline{8-11}
\multicolumn{1}{c|}{} &  & (0.10) & (15.90) & (5.39) & \bf(0.06) &  & (3.48) & (15.00) & (15.34) & \bf(1.72) &  \\ \cline{2-6} \cline{8-11}
\multicolumn{1}{c|}{} & \multirow{2}{*}{20} & 2.98 & 4.38 & 4.40 & \bf 1.12 &  & 7.54 & 6.63 & 11.76 & \bf 1.77 &  \\ %\cline{3-6} \cline{8-11}
\multicolumn{1}{c|}{} &  & (0.15) & (3.95) & (5.11) & \bf(0.09) &  & (2.77) & (7.94) & (6.60) & \bf(0.49) &  \\ \cline{2-6} \cline{8-11}
\multicolumn{1}{c|}{} & \multirow{2}{*}{40} & 3.90 & 10.11 & 11.96 & \bf 1.00 &  & 5.76 & 5.53 & 7.82 & \bf 1.64 &  \\ %\cline{3-6} \cline{8-11}
\multicolumn{1}{c|}{} &  & (0.22) & (15.74) & (9.56) & \bf(0.29) &  & (0.90) & (2.51) & (10.73) & \bf(0.18) &  \\ \midrule
\multicolumn{1}{c|}{\multirow{6}{*}{CIFAR10}} & \multirow{2}{*}{10} & 34.60 & 77.01 & 77.56 & \bf 18.56 & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}32.85\\ (1.03)\end{tabular}} & 70.65 & 81.12 & 81.55 & \bf 42.92 & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}58.62\\ (8.63)\end{tabular}} \\ %\cline{3-6} \cline{8-11}
\multicolumn{1}{c|}{} &  & (0.30) & (5.02) & (8.71) & \bf(0.04) &  & (2.38) & (5.41) & (7.09) & \bf(3.02) &  \\ \cline{2-6} \cline{8-11}
\multicolumn{1}{c|}{} & \multirow{2}{*}{20} & 42.06 & 78.74 & 84.18 & \bf 19.66 &  & 63.53 & 65.51 & 70.51 & \bf 35.24 &  \\ %\cline{3-6} \cline{8-11}
\multicolumn{1}{c|}{} &  & (1.63) & (6.96) & (5.95) & \bf(0.30) &  & (1.24) & (13.16) & (7.66) & \bf(0.98) &  \\ \cline{2-6} \cline{8-11}
\multicolumn{1}{c|}{} & \multirow{2}{*}{40} & 46.02 & 73.75 & 78.65 & \bf 20.31 &  & 53.78 & 65.72 & 60.23 & \bf 31.43 &  \\ %\cline{3-6} \cline{8-11}
\multicolumn{1}{c|}{} &  & (0.67) & (4.78) & (6.91) & \bf(0.69) &  & (0.13) & (3.93) & (5.71) & \bf(1.72) &  \\ \midrule
\end{tabular}%
}
\end{table}
\fi
% Old table
% \begin{table}[t]
% \centering
% \caption{Quantitative comparison of our method with other state-of-the-art unlabeled data learning algorithm within a FL system on benchmark datasets.}
% \label{tb:comp_sota}
% \scalebox{0.85}{
% \begin{tabular}{c|p{1cm}<{\centering}|p{1cm}<{\centering}|ccc|c|c}
% \toprule
% Dataset&Clients&Sets&FedPL&FedLLP&FedLLP-VAT&FedUU&Supervised\\
% \hline
% \multirow{5}{*}{MNIST} & 5 & 10 & 63.21 (11.66) & 26.58 (7.02) & 42.68 (11.00) & 1.52 (0.26) & \multirow{5}{*}{0.44 (0.07)}
%  \\
%  &5 & 20 & 46.53 (5.54) & 14.02 (13.99) & 10.56 (16.14) & 1.41 (0.19)
%  \\
%  &5 & 30 & 46.17 (1.90) & 7.40 (11.20) & 4.30 (5.60) & 1.41 (0.15)
%  \\
%  &5 & 40 & 39.19 (10.57) & 28.10 (5.25) & 13.42 (2.38) & 1.39 (0.17)
%  \\
%  &5 & 50 & 28.30 (10.56) & 24.55 (14.42) & 31.28 (13.74) & 1.20 (0.28)
%  \\\hline
%  \multirow{5}{*}{CIFAR10} & 5 & 10 & 82.57 (1.51) & 81.92 (7.05) & 79.91 (7.01) & 38.41 (5.40) &
%  \multirow{5}{*}{13.03 (0.45)}
%  \\
%  &5 & 20 & 79.81 (1.65) & 73.07 (4.87) & 70.97 (13.68) & 36.28 (4.10)
%  \\
%  &5 & 30 & 81.14 (0.47) & 61.35 (13.18) & 65.62 (5.13) & 38.36 (4.94)
%  \\
%  &5 & 40 & 79.24 (1.44) & 66.44 (20.13) & 63.16 (10.77) & 33.27 (0.64)
%  \\
%  &5 & 50 & 78.63 (0.74) & 59.39 (15.05) & 64.11 (10.90) & 34.10 (3.43)
%  \\
% \bottomrule
% \end{tabular}
% }
% \end{table}


% \textbf{Overviews:}
% we present a comprehensive investigation on the properties of the proposed FedUU approach, including: (1) effects of accessible clients amount; (2) behavior with respect to the choices of local update epochs; (3) effects of batch size; (4) comparison to state of the art; (5) robustness of our model under noise.

\textbf{Baselines:}
% To validate the effectiveness of our method, we conduct several baselines with state-of-the-art LLP methods \Xiaoxiao{To Do: Ask Nan about the suitable wording.} 
% We compare our method with the following baseline methods: 
(1) Federated Pseudo Labeling (FedPL) \citep{diao2021semifl}: 
% we denote the most class in a set as the label of all the samples in this set with mixup strategy; 
at each client of a FedAvg system, we choose the label with the largest class prior in a U set as the pseudo label for all the data in this set. During local training, these pseudo labels are boosted by \emph{Mixup} \citep{zhang2017mixup} high-confidence data and low-confidence data, where the confidence is given by model predictions.
(2) Federated LLP (FedLLP) \citep{dulac2019deep}: 
% we update each client model by minimizing the distance between the ground truth label proportion and the predicted label proportion, and aggregate them using FedAvg; 
each client model is updated by minimizing the distance between the ground truth label proportion and the predicted label proportion, and we aggregate them using FedAvg.
(3) FedLLP with Virtual Adversarial Training (FedLLP-VAT) \citep{tsai2020learning}: a consistency term is added to FedLLP as regularization for optimizing client model in FedAvg.
%We also train the model in a supervised manner with 10\% training data following the comparison setting in the classical unsupervised classification literature \citep{chen2020simple} under a FedAvg system. 
(4) FedAvg with 10\% labeled data (FedAvg 10\%): following \citet{chen2020simple},
% the unsupervised classification literature \citep{chen2020simple}, 
we also compare with supervised learning based on FedAvg using 10\% fully labeled data.
% total data samples with true labels. 
The detailed baseline settings are depicted in Appendix~\ref{app:exp}. 

\textbf{Results:}
The experimental results of our method and baselines on two benchmark datasets under IID and Non-IID settings are reported in Table \ref{tb:comp_sota},
where
% The results are reported in 
the mean error (std) 
% format 
over clients 
% with three independent runs.
based on 3 independent runs are shown.
Given the limited number of total data available in the benchmark datasets, we compare our method with baselines in an FL system with five clients and vary the number of U sets $M \in \{10, 20, 40\}$ at each client. In this regard, each set contains a sufficient number of data samples to train the model.

%As shown in Table~\ref{tb:comp_sota}, 
% Note 
Our observations are as follows.
First, the proposed FedUL method outperforms other baseline methods by a large margin under both IID and Non-IID settings. 
% Moreover, we have the following observations.
Second, when varying the number of sets $M\in \{10, 20, 40\}$, 
FedUL not only achieves lower classification error but also shows more stable performance compared to baselines.
Third, as we use FedAvg as the default aggregation strategy for all the methods, 
% as expected, FedUL, FedPL, and FedAvg degrade model performance under inter client Non-IID setting. 
the performances of FedUL, FedPL, and FedAvg all degrade under the inter-client Non-IID setting, as expected. 
The error rates of FedLLP and FedLLP-VAT are high and unstable, 
% probably due to the limitation of EPRM methods.
which demonstrates that the EPRM based methods are inferior as discussed in Section~\ref{sec:intro}.

%\iffalse
% Specially, empirical proportion risk based methods, i.e., FedLLP and FedLLP-VAT are suffering from its own limitation which produce very unstable results.
% Within the classification risk based methods, we can summarize our observations as follows:
% \begin{itemize}
%     \item As there are numerous samples with incorrect pseudo labels used for training in FedPL, its performance is limited.
%     \item Our proposed method advances in learning from surrogate labeled data. It not only outperforms empirical proportion risk based method, but also achieves much lower classification error compared with FedPL and FedAvg consistently on 10, 20 and 40 sets.
%     \item Both FedPL and FedAvg suffer a lot from inter client Non-IID setting, we can see their performance drop by a very large margin. However, in this very challenging Non-IID setting, our method can still work well.
% \end{itemize}
% \fi
% From Table \ref{tb:comp_sota}, we can observe that

% \textbf{Comparison with State-of-the-art:}
% To further validate the effectiveness of our method, we compare our method with several state-of-the-art LLP methods under a FL system: (1) Pseudo labeling \citep{diao2021semifl}; (2) LLP \citep{dulac2019deep}; (3) LLP-VAT \citep{tsai2020learning}; (4) FedAvg \citep{mcmahan2017communication}. We also train the model in a fully supervised manner under a FedAvg system
% From Table \ref{tb:comp_sota}, we can 


% \textbf{Robustness with Noise:}
% Table \ref{tb:noise_robustness}


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{paper/figures/comp_sota.pdf}
%     \caption{Comparison with SOTA on training loss and error rate.}
%     \label{fig:comp_sota}
% \end{figure}

\subsection{Ablation Studies}
In the following, we present a comprehensive investigation on the ablation studies of the proposed FedUL method on MNIST benchmark.

\textbf{Robustness with Noisy Class Priors:}
To investigate the robustness of our method, we further apply FedUL in a noisy environment. 
Specifically, we perturb the class priors $\pi_{c}^{m,k}$ by a random noise $\gamma$,
and let the method treat the noisy class prior $\tilde{\pi}_{c}^{m,k} = \pi_{c}^{m,k} \cdot ((2\epsilon - 1)\gamma + 1)$, where $\gamma$ uniform randomly take values in $[0, 1]$ and $\epsilon \in \{0, 0.2, 0.4, 0.8, 1.6\}$,
as the true $\pi_{c}^{m,k}$ during the whole learning process.
% In this case, the noisy class prior $\tilde{\pi}_{c}^{m,k} = \pi_{c}^{m,k} \cdot ((2\epsilon - 1)\gamma + 1)$, where $\gamma$ uniform randomly take values in $[0, 1]$ and $\epsilon \in \{0, 0.2, 0.4, 0.8, 1.6\}$, so that the method would treat noisy $\tilde{\pi}_{c}^{m,k} \in [\pi_{c}^{m,k}(1-\gamma), \pi_{c}^{m,k}(1+\gamma)]$ as the true $\pi_{c}^{m,k}$ during the whole learning process. 
Note that we tailor the noisy $\tilde{\pi}_{c}^{m,k}$ if it surpasses the range. 
We conduct experiments with five clients and ten U sets at each client. 
The experimental setup is the same as before except for the replacement of $\pi_{c}^{m,k}$. 
% Here we conduct experiments with five clients and ten U sets at each client. 
From Figure \ref{fig:mnist_ablation_a}, we can see that FedUL performs stably even with some challenging noise perturbations (see when noise ratio $\epsilon>0$).

\textbf{Effects of the Number of Accessible Non-IID U Data:}
% Experiments with 5k, 10k, 15k, 20k and 25k samples.
The purpose of FL is utilizing more data to empower model performance. While how unlabeled data, especially unlabeled Non-IID data, can contribute to FL model performance needs investigation.
To this end, we analyze the effects of the number of accessible Non-IID U data.
% theoretical result \Zhao{I am not sure which one to ref} that more unlabeled Non-IID data can be helpful for FL. 
% In this regard, 
We set each client with $n_c=500$ samples $\forall c \in [C]$ and conduct experiments by changing the amount of Non-IID U data by increasing the number of clients $C\in\{10, 20, 30, 40, 50\}$. 
% Here, we fix 
% % all of experiments with 
% $B=128$ and $E=1$.  
As shown in Figure \ref{fig:mnist_ablation_b}, 
% it is obvious that 
the model performance improves by a large margin as the number of accessible Non-IID U data increases by using our proposed FedUL method.
% \Xiaoxiao{Zhao: due to the current scale of y-axis, the `large margin' is not obvious. I can adapt the range of y-axis.}

\textbf{Analysis of Local Updating Epochs:}
% Experiments with 1, 4 and 16 local update steps.
The frequency of aggregation may sometimes influence the model performance in an FL system. We would like to explore if FedUL is stable when the local clients are updated with different local epochs $E$. %($E\textgreater1$). 
In Figure \ref{fig:mnist_ablation_c}, we explore $E\in\{1, 2, 4, 8, 16\}$ with fixed $B=128$ and $C=5$. The results demonstrate that with different $E$, the performances of FedUL are reasonably stable.
% with almost the same performance.

\textbf{Effects of Batch Size:}
The training batch size is always an important factor in machine learning tasks, especially in an FL system. Hence here, we study how batch size affects our model performance.
% in an FL system. 
Specifically, we train the model using different batch sizes~$B\in\{16, 64, 128, 512, \infty\}$ with fixed $E=1$ and $C=5$. Here $B=\infty$ stands for loading all of the training samples 
% from the training data 
into a single batch. The results in Figure \ref{fig:mnist_ablation_d} indicate that FedUL can effectively work under a wide range of batch sizes.
% Experiments with 16, 128 and $\infty$ training batch size.
% Figure \ref{fig:mnist_ablation} (c)

\begin{figure}[t]
\centering

\subfigure[]{
\begin{minipage}[t]{0.24\textwidth}
\label{fig:mnist_ablation_a}
\centering
\includegraphics[width=\textwidth]{figures/mnist_n.pdf}
\end{minipage}
}%
\subfigure[]{
\begin{minipage}[t]{0.24\textwidth}
\label{fig:mnist_ablation_b}
\centering
\includegraphics[width=0.97\textwidth]{figures/mnist_c.pdf}
\end{minipage}%
}%
\subfigure[]{
\begin{minipage}[t]{0.24\textwidth}
\label{fig:mnist_ablation_c}
\centering
\includegraphics[width=\textwidth]{figures/mnist_e.pdf}
\end{minipage}%
}%
\subfigure[]{
\begin{minipage}[t]{0.24\textwidth}
\label{fig:mnist_ablation_d}
\centering
\includegraphics[width=\textwidth]{figures/mnist_b.pdf}
\end{minipage}%
}%

\vspace{-3mm}
\centering
\caption{Ablation studies on MNIST under a Non-IID FL system. (a) Study on the robustness of our method with noisy class priors. (b) Effects of the number of accessible Non-IID U data. (c) Analysis of local updating epochs. (d) Effects of training batch size.
% \Xiaoxiao{Zhao: Pls add the values of mean and std to the figures.} 
% \Xiaoxiao{The pattern shown in (b) (c) is not clear with 3 points. Do you still have time to add batchsize = 64 and local=8. But this is not a task with high priority if you have not finished the others.}\Zhao{Running now :)}
}
\label{fig:mnist_ablation}
% \vspace{-5mm}
\end{figure}

% \iffalse
% \fi

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\iffalse
\begin{table}[t]
\normalsize
\renewcommand\arraystretch{1.5}
\centering
\caption{\small Quantitative comparison of our method with other state-of-the-art unlabeled data learning algorithm within a Non-IID FL system with five hospitals (H) on real-world intracranial hemorrhage detection dataset. Results of three runs are reported in mean(std) format. The best accuracy is highlighted in boldface.}
\label{tb:real_data}
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{0.3cm}<{\centering}|c|c|c|c|c|c|c|c|c|c|p{0.6cm}<{\centering}|p{0.6cm}<{\centering}|p{0.6cm}<{\centering}|p{0.6cm}<{\centering}|p{0.6cm}<{\centering}}
\toprule
 & \multicolumn{5}{c|}{FedPL} & \multicolumn{5}{c|}{\textbf{FedUL (ours)}} & \multicolumn{5}{c}{FedAvg 10\%} \\ \hline \hline
\multicolumn{1}{l|}{Sets} & H1 & H2 & H3 & H4 & H5 & H1 & H2 & H3 & H4 & H5 & H1 & H2 & H3 & H4 & H5 \\ \hline
\multirow{2}{*}{12} & 44.69 & 46.42 & 46.29 & 47.55 & 46.53 & \textbf{40.26} & \textbf{40.35} & \textbf{39.31} & \textbf{39.72} & \textbf{39.43} & \multirow{6}{*}{\begin{tabular}[l]{@{}l@{}}46.79\\ (1.91)\end{tabular}} & \multirow{6}{*}{\begin{tabular}[l]{@{}l@{}}46.44\\ (0.78)\end{tabular}} & \multirow{6}{*}{\begin{tabular}[l]{@{}l@{}}47.19\\ (1.05)\end{tabular}} & \multirow{6}{*}{\begin{tabular}[l]{@{}l@{}}47.29\\ (1.93)\end{tabular}} & \multirow{6}{*}{\begin{tabular}[l]{@{}l@{}}46.20\\ (1.61)\end{tabular}} \\
 & (4.28) & (4.35) & (1.83) & (2.84) & (2.40) & (1.39) & (1.10) & (1.10) & (0.64) & (1.42) &  &  &  &  &  \\ \cline{1-11}
\multirow{2}{*}{24} & 42.71 & 42.18 & 42.30 & 41.79 & 41.46 & \textbf{32.27} & \textbf{30.99} & \textbf{31.29} & \textbf{31.72} & \textbf{31.27} &  &  &  &  &  \\
 & (2.97) & (3.00) & (1.28) & (1.98) & (0.53) & (2.71) & (2.03) & (1.05) & (1.23) & (1.58) &  &  &  &  &  \\ \cline{1-11}
\multirow{2}{*}{48} & 41.44 & 40.38 & 41.06 & 41.44 & 40.26 & \textbf{31.48} & \textbf{30.90} & \textbf{31.16} & \textbf{31.55} & \textbf{30.57} &  &  &  &  &  \\
 & (3.04) & (1.38) & (2.88) & (1.78) & (2.35) & (2.25) & (0.88) & (0.84) & (0.58) & (1.30) &  &  &  &  &  \\ \bottomrule
\end{tabular}%
}
\end{table}
\fi

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\iffalse
\begin{table}[t]
\renewcommand\arraystretch{1.2}
\centering
\caption{\small Quantitative comparison of our method with other state-of-the-art unlabeled data learning algorithm within a Non-IID FL system with five hospitals (H) on real-world intracranial hemorrhage detection dataset. Results of three runs are reported in mean(std) format. }
\label{tb:real_data}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{c|ccc|ccc|c}
\toprule
 & \multicolumn{3}{c|}{FedPL} & \multicolumn{3}{c|}{\textbf{FedUL (ours)}} & FedAvg 10\% \\ \hline \hline
Sets & 12 & 24 & 48 & 12 & 24 & 48 & - \\ \hline
H1 & 44.69(4.28) & 42.71(2.97) & 41.44(3.04) & \textbf{40.26(1.39)} & \textbf{32.27(2.71)} & \textbf{31.48(2.25)} & 46.79(1.91) \\ \hline
H2 & 46.42(4.35) & 42.18(3.00) & 42.06(1.38) & \textbf{40.35(1.10)} & \textbf{30.99(2.03)} & \textbf{30.90(0.88)} & 46.44(0.78) \\ \hline
H3 & 46.29(1.83) & 42.30(1.28) & 41.06(2.88) & \textbf{39.31(1.10)} & \textbf{31.29(1.05)} & \textbf{31.16(0.84)} & 47.19(1.05) \\ \hline
H4 & 47.55(2.84) & 41.79(1.98) & 41.44(1.78) & \textbf{39.72(0.64)} & \textbf{31.72(1.23)} & \textbf{31.55(0.58)} & 47.29(1.93) \\ \hline
H5 & 46.53(2.40) & 41.46(0.53) & 40.26(2.35) & \textbf{39.43(1.42)} & \textbf{31.27(1.58)} & \textbf{30.57(1.30)} & 46.20(1.61) \\ \bottomrule
\end{tabular}%
}
\end{table}
\fi
% old real date table
% \begin{table}[t]
% \renewcommand\arraystretch{1.2}
% \centering
% \caption{Quantitative comparison of our method with other state-of-the-art unlabeled data learning algorithm within a Non-IID FL system with 5 clients on real world intracranial hemorrhage setection dataset (Mean errors (standard deviations)). Please note that `Avg 10\%' means using 10\% labeled data following \cite{chen2020simple}.}
% \label{tb:real_data}
% \scalebox{0.93}{
% \begin{tabular}{p{1cm}<{\centering}|c|c|c}
% \toprule
% Sets&FedPL&FedUL&FedAvg 10\%\\
% \hline
% % 5 & 6 &  & &  & 40.55
% 12 & 46.84 (3.06) & \bf 39.81 (0.65) &\multirow{3}{*}{46.78 (0.95)} 
%  \\
% 24 & 42.11 (1.87) & \bf \bf 31.53 (1.58)
%  \\
% 48 & 40.92 (2.45) & \bf 31.14 (0.62)
%  \\
% % 5 & 96 & &  &  & 42.81
% \bottomrule
% \end{tabular}
% }
% \end{table}

\subsection{Case Study on Real-world Problem}
To demonstrate the feasibility of our proposed FedUL scheme to the real problem, we test FedUL on a medical application for the diagnosis of brain disease. In the rest of this section, we introduce the problem formulation, data and setting, and then discuss the results.

\textbf{Real Problem Formulation:}
For the real-world scenario, we consider a clinical setting for disease classification in $C$ different healthcare systems. Suppose each healthcare system has $M$ hospitals located in different regions, each associated with unique class priors due to population diversities. Medical data are not shareable between the healthcare systems for privacy reasons. We assume patient-wise diagnosis information is unavailable, but each hospital provides the prevalence of these patients (i.e.,
% label proportions 
class priors of the disease classes). 

%Due to the privacy regulations on patient data, all the medical data are not shareable between the hospitals. Further, we can not learn detailed patient-wise diagnosis information. Instead, each hospital branch only provides the prevalence of these patients (a.k.a, label proportions of the disease classes). These hospitals aim to collaboratively train a disease classification model using FL. In this scenario, we formulate an unsupervised FL problem with label proportion available,  where each hospital is treated as a client, and its regional branches are treated as its U sets. Given a hospital indexed by $i$ has branches in $M$ regions, we can access the prevalence of patients in branch $m\in[M]$, $\pi_c^m$ as class-prior. 
%months data from every hospital, and for every month we can access the prevalence $\pi_c^m$ of patients. 
% \Xiaoxiao{Zhao, please change the footnote to citation. You can google how to make website bib for latex.} 

\begin{table}[t]
\renewcommand\arraystretch{1.1}
\centering
\caption{Quantitative comparison of our method with the baseline methods for the five healthcare systems (HS) using the real-world intracranial hemorrhage detection dataset. Results of three runs are reported in mean error (std) format. The best methods are highlighted in boldface.}
\vspace{1ex}
\label{tb:real_data}
%\resizebox{0.9\textwidth}{!}{% Nan: ur can adjust the table by tuning here
\scalebox{0.88}{
\begin{tabular}{p{1.3cm}<{\centering}|c|ccccc}
\toprule
Hospitals &Method&HS 1&HS 2&HS 3& HS 4&HS 5\\
\hline
\multirow{2}{*}{12} & FedPL & 44.69 (4.28) & 46.42 (4.35) & 46.29 (1.83) & 47.55 (2.84) & 46.53 (2.40)
 \\
 & \bf FedUL (ours) & \bf 40.26 (1.39) & \bf 40.35 (1.10) & \bf 39.31 (1.10) & \bf 39.72 (0.67) & \bf 39.43 (1.42)
 \\
%  & FedAvg 10\% & 
%  \\
 \hline
\multirow{2}{*}{24} & FedPL & 42.71 (2.97) & 42.18 (3.00) & 42.30 (1.28) & 41.79 (1.98) & 41.46 (0.53)
 \\
 & \bf FedUL (ours) & \bf 32.27 (2.71) & \bf 30.99 (2.03) & \bf 31.29 (1.05) & \bf 31.72 (1.23) & \bf 31.37 (1.58) 
 \\
%  & FedAvg 10\% & 
%  \\
 \hline
\multirow{2}{*}{48} & FedPL & 41.44 (3.04) & 40.38 (1.38) & 41.06 (2.88) & 41.44 (1.78) & 40.26 (2.35)
 \\
 & \bf FedUL (ours) & \bf 31.48 (2.25) & \bf 30.92 (0.88) & \bf 31.16 (0.84) & \bf 31.55 (0.58) & \bf 30.57 (1.37)
 \\
 \hline
 - & FedAvg 10\% & 46.79 (1.91) & 46.44 (0.78) & 47.19 (1.05) & 47.29 (1.93) & 46.20 (1.61)
 \\
\bottomrule
\end{tabular}
}
\end{table}

\begin{figure}[t]
% \vspace{-1mm}
\centering
\includegraphics[width=0.9\textwidth]{figures/braindata.pdf}
\vspace{-1mm}
\centering
\caption{Example samples of each class in the distributed medical dataset \citep{flanders2020construction}. 
% (a) Normal ; (b) Epidural; (c) Intraparenchymal; (d) Intraventricular; (e) Subarachnoid; (f) Subdural.
}
\label{fig:braindata}
% \vspace{-3mm}
\end{figure}

\textbf{Dataset and Settings:} We use the RSNA Intracranial Hemorrhage Detection dataset \citep{flanders2020construction}, which contains large-scale Magnetic Response Image (MRI) data from several hospitals (see Figure~\ref{fig:braindata}), to simulate this real-world scenario. 
% The dataset contains large-scale Magnetic Response Image (MRI) data from several hospitals.
%in which some of them are diagnosed as intracranial hemorrhage. 
%Intracranial hemorrhage, described as bleeding that occurs inside the cranium, is a severe health problem and depends on the patient's ethnicity. For example, age is a directly associated factor~\citep{camacho2015role}. Thus, considering age distributions vary in different regions, this dataset naturally fits into our setting.
There are $106k$ samples in the dataset belonging to six classes, including five types of intracranial hemorrhage (Epidural, Intraparenchymal, Intraventricular, Subarachnoid, and Subdural) and healthy control type. %We model a more realistic and challenging Non-IID setting on this dataset.  Based on this formulation, 
We model an FL system with five healthcare systems (i.e., clients). Each healthcare system contains $21.2k$ data samples. To show the effect on the number of samples in each U set, we vary the number of hospitals (i.e., sets) $M =12$, $24$, and $48$ in each system. Here we generate each $\pi_{c}^{m,k}$ for the $k$-th class in $m$-th U set at $c$-th client from range $[0.1,0.9]$
% for all the U sets 
and check that the generated class priors are not all identical.
%As this dataset is naturally in a Non-IID pattern, so we do not impose class-prior shift.
For model training, we use the cross-entropy loss and Adam \citep{kingma2014adam} optimizer with a learning rate of $1e-4$ and train 100 rounds. We use ResNet18 \citep{he2016deep} as backbone for this experiment.
% \Xiaoxiao{How we generate $\pi$, what is the arch? what is training strategy.}

\textbf{Results and Analysis:}
As indicated in our proof-of-concept (Table~\ref{tb:comp_sota}), FedPL consistently outperforms the other two LLP baselines, i.e., FedLLP and FedLLP-VAT.
Here we focus on comparing FedUL with FedPL.
The supervised baseline FedAvg
% in supervised learning 
with 10\% fully labeled data is also included for reference. We report the results of each hospital in mean error (std) format over three runs in Table \ref{tb:real_data}. 
% From Table \ref{tb:real_data}, 
We can see that our proposed FedUL method consistently outperforms FedPL and FedAvg 10\% for all the hospitals and under different set number settings. The superiority of FedUL in this challenging real-world FL setting further indicates the effectiveness and robustness of our algorithm. These results are inspiring and bring the hope of deploying FedUL to the healthcare
field, where data are often very costly to be labeled, heterogeneous, and distributed.




















==> Federated Learning with Only Unlabeled Datasets final/sections/experimental_details.tex <==
\newpage
\section{Experimental details}
\label{app:exp}
We illustrate our model architectures and training details of the benchmark and real-world experiments in this section.

\subsection{Model Architecture}

For our benchmark experiment on MNIST, we use a six-layer convolutional neural network. The network details are listed in Table \ref{tab:model_mnist}. For our benchmark experiment on CIFAR10 and real-world experiment, we use ResNet18 as our backbone. The network details are listed in Table \ref{tab:model_cifar10}.

\begin{table}[ht]
\renewcommand\arraystretch{1.2}
\centering
% \resizebox{0.5\textwidth}{!}{%
\scalebox{0.99}{
\begin{tabular}{l|cccc}
\toprule
\multicolumn{1}{c|}{\multirow{1}{*}{Layer}} & \multicolumn{4}{c}{Details} \\ \hline
\multicolumn{1}{c|}{\multirow{1}{*}{1}}& \multicolumn{4}{c}{Conv2D(3, 64, 5, 1, 2), BN(64), ReLU, MaxPool2D(2, 2)} \\\hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(64), ReLU, MaxPool2D(2, 2)} \\ \hline
\multicolumn{1}{c|}{\multirow{1}{*}{2}}& \multicolumn{4}{c}{Conv2D(64, 64, 5, 1, 2), BN(64), ReLU, MaxPool2D(2, 2)} \\\hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(64), ReLU, MaxPool2D(2, 2)} \\ \hline
\multicolumn{1}{c|}{\multirow{1}{*}{3}}& \multicolumn{4}{c}{Conv2D(64, 128, 5, 1, 2), BN(128), ReLU} \\\hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(128), ReLU} \\ \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{3}}& \multicolumn{4}{c}{Conv2D(64, 128, 5, 1, 2)} \\
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(128), ReLU} \\ \hline
\multicolumn{1}{c|}{\multirow{1}{*}{4}}& \multicolumn{4}{c}{FC(6272, 2048), BN(2048), ReLU} \\\hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(2048), ReLU} \\ \hline
\multicolumn{1}{c|}{\multirow{1}{*}{5}}& \multicolumn{4}{c}{FC(2048, 512), BN(512), ReLU} \\\hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(512), ReLU} \\ \hline
\multicolumn{1}{c|}{\multirow{1}{*}{6}}& \multicolumn{4}{c}{FC(512, 10)} \\ \bottomrule
\end{tabular}%
}
\caption{Model architecture of the benchmark experiment on MNIST. For convolutional layer (Conv2D), we list parameters with sequence of input and output dimension, kernel size, stride and padding. For max pooling layer (MaxPool2D), we list kernel and stride. For fully connected layer (FC), we list input and output dimension. For BatchNormalization layer (BN), we list the channel dimension.}
\label{tab:model_mnist}
\end{table}

\begin{table}[h]
\renewcommand\arraystretch{1.2}
\centering
% \resizebox{0.4\textwidth}{!}{%
\scalebox{0.99}{
\begin{tabular}{l|cccc}
\toprule
\multicolumn{1}{c|}{\multirow{1}{*}{Layer}} & \multicolumn{4}{c}{Details} \\ \hline
\multicolumn{1}{c|}{\multirow{1}{*}{1}}& \multicolumn{4}{c}{Conv2D(3, 64, 7, 2, 3), BN(64), ReLU} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(64), ReLU} \\ \hline
% layer1
\multicolumn{1}{c|}{\multirow{1}{*}{2}}& \multicolumn{4}{c}{Conv2D(64, 64, 3, 1, 1), BN(64), ReLU} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(64), ReLU} \\ \hline
\multicolumn{1}{c|}{\multirow{1}{*}{3}}& \multicolumn{4}{c}{Conv2D(64, 64, 3, 1, 1), BN(64)} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(64)} \\ \hline

\multicolumn{1}{c|}{\multirow{1}{*}{4}}& \multicolumn{4}{c}{Conv2D(64, 64, 3, 1, 1), BN(64), ReLU} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(64), ReLU} \\ \hline
\multicolumn{1}{c|}{\multirow{1}{*}{5}}& \multicolumn{4}{c}{Conv2D(64, 64, 3, 1, 1), BN(64)} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(64)} \\ \hline

% layer2
\multicolumn{1}{c|}{\multirow{1}{*}{6}}& \multicolumn{4}{c}{Conv2D(64, 128, 3, 2, 1), BN(128), ReLU} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(128), ReLU} \\ \hline
\multicolumn{1}{c|}{\multirow{1}{*}{7}}& \multicolumn{4}{c}{Conv2D(128, 128, 3, 1, 1), BN(64)} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(64)} \\ \hline

% downsample
\multicolumn{1}{c|}{\multirow{1}{*}{8}}& \multicolumn{4}{c}{Conv2D(64, 128, 1, 2, 0), BN(128)} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(128)} \\ \hline

\multicolumn{1}{c|}{\multirow{1}{*}{9}}& \multicolumn{4}{c}{Conv2D(128, 128, 3, 1, 1), BN(128), ReLU} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(128), ReLU} \\ \hline
\multicolumn{1}{c|}{\multirow{1}{*}{10}}& \multicolumn{4}{c}{Conv2D(128, 128, 3, 1, 1), BN(64)} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(64)} \\ \hline

% layer3
\multicolumn{1}{c|}{\multirow{1}{*}{11}}& \multicolumn{4}{c}{Conv2D(128, 256, 3, 2, 1), BN(128), ReLU} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(128), ReLU} \\ \hline
\multicolumn{1}{c|}{\multirow{1}{*}{12}}& \multicolumn{4}{c}{Conv2D(256, 256, 3, 1, 1), BN(64)} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(64)} \\ \hline

% downsample
\multicolumn{1}{c|}{\multirow{1}{*}{13}}& \multicolumn{4}{c}{Conv2D(128, 256, 1, 2, 0), BN(128)} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(128)} \\ \hline

\multicolumn{1}{c|}{\multirow{1}{*}{14}}& \multicolumn{4}{c}{Conv2D(256, 256, 3, 1, 1), BN(128), ReLU} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(128), ReLU} \\ \hline
\multicolumn{1}{c|}{\multirow{1}{*}{15}}& \multicolumn{4}{c}{Conv2D(256, 256, 3, 1, 1), BN(64)} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(64)} \\ \hline

% layer4
\multicolumn{1}{c|}{\multirow{1}{*}{16}}& \multicolumn{4}{c}{Conv2D(256, 512, 3, 2, 1), BN(512), ReLU} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(512), ReLU} \\ \hline
\multicolumn{1}{c|}{\multirow{1}{*}{17}}& \multicolumn{4}{c}{Conv2D(512, 512, 3, 1, 1), BN(512)} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(512)} \\ \hline

% downsample
\multicolumn{1}{c|}{\multirow{1}{*}{18}}& \multicolumn{4}{c}{Conv2D(256, 512, 1, 2, 0), BN(512)} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(512)} \\ \hline

\multicolumn{1}{c|}{\multirow{1}{*}{19}}& \multicolumn{4}{c}{Conv2D(512, 512, 3, 1, 1), BN(512), ReLU} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(512), ReLU} \\ \hline
\multicolumn{1}{c|}{\multirow{1}{*}{20}}& \multicolumn{4}{c}{Conv2D(512, 512, 3, 1, 1), BN(512)} \\ \hline
% \multicolumn{1}{c|}{} &\multicolumn{4}{c}{BN(512)} \\ \hline

\multicolumn{1}{c|}{\multirow{1}{*}{21}}& \multicolumn{4}{c}{AvgPool2D}\\ \hline

\multicolumn{1}{c|}{\multirow{1}{*}{22}}& \multicolumn{4}{c}{FC(512, 10)} \\ \bottomrule
\end{tabular}%
}
\caption{Model architecture of the benchmark experiment on CIFAR10. For convolutional layer (Conv2D), we list parameters with sequence of input and output dimension, kernel size, stride and padding. For max pooling layer (MaxPool2D), we list kernel and stride. For fully connected layer (FC), we list input and output dimension. For BatchNormalization layer (BN), we list the channel dimension.}
\label{tab:model_cifar10}
\end{table}


\subsection{Training Details}
\paragraph{Benchmark Experiments:}
We implement all the methods by PyTorch and conduct all the experiments on an NVIDIA TITAN X GPU. 
Please note for all experiments, we split 20\% original data for validation and model selection. During training process, we use Adam optimizer with learning rate $1e-4$ and the cross-entropy loss. We set batch size to $128$ and training rounds to $100$. To avoid overfitting, we use L1 regularization. The detailed weight of L1 regularization used in benchmark experiments is shown in Table \ref{tb:l1norm_weight_benchmark}.
The detailed number of samples at each client for MNIST and CIFAR10 under IID and Non-IID setting is given in Table \ref{tab:mnist_detailed} and Table \ref{tab:cifar_detailed}, respectively.

\begin{table}[ht]
\renewcommand\arraystretch{1.1}
  \centering
  \caption{Detailed weight of L1 regularization used in benchmark experiments.}
  \scalebox{0.95}{
    \begin{tabular}{c|ccc|ccc}
    \toprule
    Dataset & \multicolumn{3}{c|}{MNIST} & \multicolumn{3}{c}{CIFAR10} \\
    \hline
    Sets  & 10    & 20    & 30    & 10    & 20    & 30 \\
    \hline
    Weight & 1e-5 & 5e-5 & 2e-6 & 2e-5 & 1e-5 & 4e-6 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tb:l1norm_weight_benchmark}%
\end{table}%



\begin{table}[ht]
\renewcommand\arraystretch{1.1}
  \centering
  \caption{Detailed number of samples at each client for MNIST benchmark}
%   \vspace{1mm}
    \scalebox{0.88}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
          & Class & 0     & 1     & 2     & 3     & 4     & 5     & 6     & 7     & 8     & 9 \\
    \hline\hline
    \multirow{5}[10]{*}{IID} & Client1 & 920   & 1098  & 970   & 972   & 945   & 893   & 898   & 1007  & 971   & 926 \\
\cline{2-12}          
& Client2 & 920   & 1098  & 970   & 972   & 945   & 893   & 898   & 1007  & 971   & 926 \\
\cline{2-12}          & Client3 & 920   & 1098  & 970   & 972   & 945   & 893   & 898   & 1007  & 971   & 926 \\
\cline{2-12}          & Client4 & 920   & 1098  & 970   & 972   & 945   & 893   & 898   & 1007  & 971   & 926 \\
\cline{2-12}          & Client5 & 920   & 1098  & 970   & 972   & 945   & 893   & 898   & 1007  & 971   & 926 \\
    \hline
    \multirow{5}[10]{*}{Non-IID} & Client1 & 4498  & 4646  & 56    & 56    & 54    & 57    & 54    & 60    & 60    & 54 \\
\cline{2-12}          & Client2 & 57    & 54    & 4425  & 4737  & 49    & 50    & 49    & 58    & 57    & 58 \\
\cline{2-12}          & Client3 & 64    & 61    & 57    & 61    & 4316  & 4217  & 54    & 53    & 58    & 57 \\
\cline{2-12}          & Client4 & 53    & 58    & 55    & 35    & 50    & 0     & 4572  & 4576  & 60    & 57 \\
\cline{2-12}          & Client5 & 57    & 58    & 61    & 0     & 60    & 0     & 19    & 54    & 4418  & 4576 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:mnist_detailed}%
\end{table}%


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[ht]
\renewcommand\arraystretch{1.1}
  \centering
  \caption{Detailed number of samples at each client for CIFAR10 benchmark}
%   \vspace{1mm}
    \scalebox{0.88}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
          & Class & airplane & automobile & bird  & cat   & deer  & dog   & frog  & horse & ship  & truck \\
    \hline
    \hline
    \multirow{5}[10]{*}{IID} & Client1 & 755   & 788   & 794   & 796   & 791   & 842   & 827   & 788   & 820   & 799 \\
\cline{2-12}          & Client2 & 755   & 788   & 794   & 796   & 791   & 842   & 827   & 788   & 820   & 799 \\
\cline{2-12}          & Client3 & 755   & 788   & 794   & 796   & 791   & 842   & 827   & 788   & 820   & 799 \\
\cline{2-12}          & Client4 & 755   & 788   & 794   & 796   & 791   & 842   & 827   & 788   & 820   & 799 \\
\cline{2-12}          & Client5 & 755   & 788   & 794   & 796   & 791   & 842   & 827   & 788   & 820   & 799 \\
    \hline
    \multirow{5}[10]{*}{Non-IID} & Client1 & 3748  & 3872  & 47    & 46    & 45    & 47    & 45    & 50    & 50    & 45 \\
\cline{2-12}          & Client2 & 48    & 45    & 3688  & 3938  & 41    & 41    & 41    & 48    & 48    & 48 \\
\cline{2-12}          & Client3 & 53    & 51    & 48    & 0     & 3597  & 3887  & 45    & 53    & 48    & 47 \\
\cline{2-12}          & Client4 & 44    & 18    & 46    & 0     & 42    & 0     & 3810  & 3813  & 50    & 48 \\
\cline{2-12}          & Client5 & 47    & 0     & 51    & 0     & 50    & 0     & 46    & 45    & 3788  & 3790 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:cifar_detailed}%
\end{table}%





We describe details of the baseline methods and corresponding hyper-parameters as follows.
\begin{itemize}
    \item FedPL \citep{diao2021semifl}: this method is based on empirical classification risk minimization. The learning objective is
    
    \begin{equation}
    \widehat{R}(\boldsymbol{f})=\frac{1}{C} \sum_{c=1}^{C} \sum_{m=1}^{M_c} \mathcal{L}_{fix} + \lambda \mathcal{L}_{mix},
    \end{equation}
     where 
    \begin{equation}
    \mathcal{L}_{\mathrm{fix}}=\ell\left(\boldsymbol{f}\left(x_{b}^{+}\right), y_{b}^{+}\right)
    \end{equation}
    is the "fix" loss.
    $(x_{b}^{+}, y_{b}^{+})$ represents for a sample $x_{b}^{+}$ with high confidence pseudo label $y_{b}^{+}$ and 
    \begin{equation}
    \left.\mathcal{L}_{\operatorname{mix}}=\lambda_{\operatorname{mix}} \cdot \ell\left(\boldsymbol{f}\left(x_{\mathrm{mix}}\right), y_{b}^{+}\right)+\left(1-\lambda_{\operatorname{mix}}\right) \cdot \ell\left(\boldsymbol{f}\left(x_{\mathrm{mix}}\right), y_{b}^{-}\right)\right)
    \end{equation}
    is the "mix" loss, in which 
    \begin{equation}
    \lambda_{\operatorname{mix}} \sim \operatorname{Beta}(a, a), \quad x_{\operatorname{mix}} \leftarrow \lambda_{\operatorname{mix}} x_{b}^{+}+\left(1-\lambda_{\operatorname{mix}}\right) x_{b}^{-}.
    \end{equation}
    $a$ is the mixup hyper-parameter and $(x_{b}^{-}, y_{b}^{-})$ represents for a sample $x_{b}^{-}$ with low confidence pseudo label $y_{b}^{-}$. Following the default implementation in \cite{diao2021semifl}, we set hyper-parameter $a=0.75$. Moreover, we set the weight of "mix" loss $\lambda=0.3$ and the confidence threshold $\tau=0.4$.
        
    
    
    \item FedLLP \citep{dulac2019deep}: this baseline method is based on empirical proportion risk minimization. The learning objective is the aggregated proportion risk, i.e.,
    \begin{equation}
    \widehat{R}(\boldsymbol{f})=\frac{1}{C} \sum_{c=1}^{C} \sum_{m=1}^{M_c} d_{\text {prop }}\left(\pi_c^{m}, \hat{\pi}_c^{m}\right)
    \end{equation}
    where $\pi_c^m$ and $\hat{\pi}_c^m$ are the true and predicted label proportions for the $m$-th U set $\mathcal{U}_{c}^m$ at the $c$-th client, $\hat{\pi}_c^m \coloneqq\frac{1}{M_c}\sum_{\bx\sim\mathcal{U}^m_c}f(\bx)$. 
    %$d_{\mathrm{prop}}$ is a distance function, e.g. cross entropy.
    For each client $c$, $d_{\mathrm{prop}}$ is defined as
    \begin{align*}
        d_{\mathrm{prop}}(\pi_c^m,\hat{\pi}_c^m) \coloneqq -\sum_{k=1}^K\pi_c^{m}\log \hat{\pi}_c^{m}.
    \end{align*}


    \item FedLLP-VAT \citep{tsai2020learning}: this method is based on empirical proportion risk minimization, integrated with a consistency regularization term. The learning objective is the aggregated proportion risk with consistency regularization, i.e.,
    \begin{equation}
    \widehat{R}(\boldsymbol{f})=\frac{1}{C} \sum_{c=1}^{C}\left(\sum_{m=1}^{M_{c}} d_{\text {prop }}\left(\pi_{c}^{m}, \widehat{\pi}_{c}^{m}\right)+\alpha \ell_{\text {cons }}(f)\right),
    \end{equation}
    where $\pi_c^m$ and $\hat{\pi}_c^m$ are the true and predicted label proportions for the $m$-th U set $\mathcal{U}_{c}^m$ at the $c$-th client, and $d_{\mathrm{prop}}$ is a distance function.
    \begin{equation}
    \ell_{\text {cons }}(f)=d_{\text {cons }}(f(\boldsymbol{x}), f(\hat{\boldsymbol{x}}))
    \end{equation}
    is the consistency loss, where $d_{\mathrm{cons}}$ is a distance function, and $\hat{\boldsymbol{x}}$ is a perturbed input from the original $\boldsymbol{x}$. Following the default implementation in their paper \citep{tsai2020learning}, we set the hyper-parameter, the weight of consistency loss $\alpha=0.05$ and the perturbation weight $\mu=6.0$ for FedLLP-VAT on CIFAR10 benchmark experiment. For MNIST benchmark, we set the hyper-parameter, the weight of consistency loss $\alpha=5e-4$ and the perturbation weight $\mu=1e-2$.


\end{itemize}





\paragraph{Real-world Experiments:} We perform a case study on the clinical task --- intracranial hemorrhage diagnosis.
% Intracranial hemorrhage, described as bleeding that occurs inside the cranium, is a severe health problem. The distribution of intracranial hemorrhage depends on the patient's ethnicity.
% such as age~\citep{camacho2015role}. Thus, considering age distributions vary in different regions, this dataset and problem naturally fits into our setting.
We use the RSNA Intracranial Hemorrhage Detection dataset \citep{flanders2020construction} (Figure~\ref{fig:braindata}), which contains large-scale Magnetic Response Image (MRI) data from several hospitals.There are $106k$ samples in the dataset belonging to six classes, including five types of intracranial hemorrhage (Epidural, Intraparenchymal, Intraventricular, Subarachnoid, and Subdural) and healthy control type. 
In our experiments, we simulate a real-world scenario with five healthcare systems (a.k.a. clients) and assume the number of hospitals (a.k.a sets) in each healthcare systems varies $M= 12$, $24$, and $48$. At first, we randomly split the whole dataset for five healthcare systems equally, so each healthcare systems is assigned $21.2k$ samples. 
Then we generate $\pi_c^m$ for $m$-th set in $c$-th client from range $[0.1,0.9]$ for all the hospitals with U data only. We check that the generated class priors are not all identical. Finally, we load samples for each the hospitals following the generated $\pi$. Detailed dataset statistics is given in Table \ref{tb:real_data_statistics}.


% \Xiaoxiao{Zhao: could you please give more details of hwo to split them into five hospitals and how to split them into sets.}

% \begin{table}[ht]

% \renewcommand\arraystretch{1.2}
%   \centering
%   \caption{Detailed statistics of RSNA Intracranial Hemorrhage Detection dataset \citep{flanders2020construction}.}
%   \scalebox{0.99}{
%     \begin{tabular}{c|cccccc}
%     \toprule
%     Type  & Healthy & Epidural & Intraparenchymal & Intraventricular & Subarachnoid & Subdural \\
%     \hline
%     Number & 30141 & 1694 & 15664 & 9878 & 16423 & 32200 \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \label{tb:real_data_statistics}%
% \end{table}%
% \Xiaoxiao{Add othe phenotype}

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
\vspace{-3mm}
\renewcommand\arraystretch{1.1}
  \centering
  \caption{Detailed number of samples in each healthcare system (HS) for real-world RSNA Intracranial Hemorrhage Detection dataset \citep{flanders2020construction}.}
  \scalebox{0.88}{
    \begin{tabular}{c|c|c|c|c|c|c}
    \toprule
    Type  & Healthy & Epidural & Intraparenchymal & Intraventricular & Subarachnoid & Subdural \\
    \hline
    HS 1 & 3726  & 221   & 2023  & 1198  & 2027  & 4005 \\
    \hline
    HS 2 & 3756  & 226   & 1923  & 1190  & 2063  & 4042 \\
    \hline
    HS 3 & 3804  & 177   & 1932  & 1266  & 2040  & 3981 \\
    \hline
    HS 4 & 3805  & 224   & 1939  & 1187  & 2074  & 3971 \\
    \hline
    HS 5 & 3711  & 198   & 1929  & 1299  & 2080  & 3983 \\
    \bottomrule
    \end{tabular}%
    }
\label{tb:real_data_statistics}%
\vspace{-3mm}
\end{table}%


 During training process, we use Adam optimizer with learning rate $1e-4$ and cross-entropy loss. We set batch size to $128$ and training rounds to $100$. To avoid overfitting, we use L1 regularization. We set the weight of L1 regularization as $2e-6$, $8e-7$ and $4e-7$ for 10, 20 and 40 sets, respectively. In real-world experiments, we use the same hyper-parameters as benchmark experiments for all methods except FedLLP-VAT. For FedLLP-VAT, we set the weight of consistency loss $\alpha=0.05$ and the perturbation weight $\mu=6.0$. 
 
 
\paragraph{Training Efficiency:}
We further evaluate the training efficiency of our method with comparison to baseline methods. The detailed one epoch training time (mean) and forward FLOPs are given in Table \ref{tb:training_time}. The computation time is evaluated on a PC with one Nvidia TITAN X GPU. We can see that our method slightly increase the forward FLOPs and can achieve higher training efficiency compared with FedPL and FedLLP-VAT.

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[h]
\renewcommand\arraystretch{1.15}
\centering
\caption{Quantitative comparison of our method with the baseline methods training epoch time and forward flops on benchmark and real-world datasets under Non-IID and IID setting.}
\label{tb:training_time}
\scalebox{0.85}{
    \begin{tabular}{c|c|c|c|c|c}
    \toprule
    \multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Non-IID Task with 5 Clients} & \multicolumn{2}{c}{IID Task with 5 Clients} \\
\cline{3-6}          &       & Computation time (s) & FLOPs (G) & Computation time (s) & FLOPs (G) \\
    \hline
    \multirow{4}{*}{MNIST} & FedPL & 3.29  & \multirow{3}{*}{0.048125312 } & 4.78  & \multirow{3}{*}{0.048125312 } \\
\cline{2-3}\cline{5-5}          & FedLLP & 1.67  &       & 2.45  &  \\
\cline{2-3}\cline{5-5}          & FedLLP-VAT & 2.10  &       & 2.87  &  \\
\cline{2-6}          & FedUL & 1.80  & 0.048125422  & 2.35  & 0.048125422  \\
    \hline
    \multirow{4}{*}{CIFAR10} & FedPL & 3.37  & \multirow{3}{*}{0.141595648 } & 5.70  & \multirow{3}{*}{0.141595648 } \\
\cline{2-3}\cline{5-5}          & FedLLP & 1.95  &       & 2.44  &  \\
\cline{2-3}\cline{5-5}          & FedLLP-VAT & 3.43  &       & 4.86  &  \\
\cline{2-6}          & FedUL & 2.63  & 0.141595758  & 3.80  & 0.141595758  \\
    \hline
    \multirow{2}{*}{Real-world} & FedPL & 32.47 & 6.937938944  & -     & - \\
\cline{2-6}          & FedUL & 32.34 & 6.937939028  & -     & - \\
    \bottomrule
    \end{tabular}}
\end{table}%



% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[h]
% \renewcommand\arraystretch{1.15}
% \centering
% \caption{Quantitative comparison of our method with the baseline methods training epoch time and forward flops on benchmark datasets under Non-IID and IID setting with 10 sets in each client.}
% \label{tb:training_time}
% \scalebox{0.85}{
%     \begin{tabular}{c|c|c|c|c|c}
%     \toprule
%     \multirow{2}[4]{*}{Dataset} & \multirow{2}[4]{*}{Method} & \multicolumn{2}{c|}{Non-IID Task with 5 Clients} & \multicolumn{2}{c}{IID Task with 5 Clients} \\
% \cline{3-6}          &       & Epoch time (s) & FLOPS (G) & Epoch time (s) & FLOPS (G) \\
%     \hline
%     \multirow{4}{*}{MNIST} & FedPL & 3.29  & \multirow{3}{*}{0.048125312 } & 4.78  & \multirow{3}{*}{0.048125312 } \\
% \cline{2-3}\cline{5-5}          & FedLLP & 1.67  &       & 2.45  &  \\
% \cline{2-3}\cline{5-5}          & FedLLP-VAT & 2.10  &       & 2.87  &  \\
% \cline{2-6}          & FedUL & 1.80  & 0.048125422  & 2.35  & 0.048125422  \\
%     \hline
%     \multirow{4}{*}{CIFAR10} & FedPL & 3.37  & \multirow{3}{*}{0.141595648 } & 5.70  & \multirow{3}{*}{0.141595648 } \\
% \cline{2-3}\cline{5-5}          & FedLLP & 1.95  &       & 2.44  &  \\
% \cline{2-3}\cline{5-5}          & FedLLP-VAT & 3.43  &       & 4.86  &  \\
% \cline{2-6}          & FedUL & 2.63  & 0.141595758  & 3.80  & 0.141595758  \\
%     \bottomrule
%     \end{tabular}}
% \end{table}%



% We use the RSNA Intracranial Hemorrhage Detection dataset \citep{flanders2020construction} (Fig.~\ref{fig:braindata}) to simulate this real-world scenario. This dataset contains large-scale Magnetic Response Image (MRI) data from several hospitals, in which some of them are diagnosed as intracranial hemorrhage. Intracranial hemorrhage, described as bleeding that occurs inside the cranium, is a severe health problem and depends on the patient's ethnicity. For example, age is a directly associated factor \citep{camacho2015role}. Thus, considering age distributions vary in different regions, this dataset naturally fits into our setting.
% There are 106000 in the dataset belonging to six classes, including five types of intracranial hemorrhage (Epidural, Intraparenchymal, Intraventricular, Subarachnoid, and Subdural) and healthy control type. We model a more realistic and challenging Non-IID setting on this dataset.  Based on this formulation, we model an FL system with five clients (w.r.t five hospitals). Each hospital contains 21200 data samples. To show the effect on the number of samples in each set, we vary $M =12$, 24 and 48 sets (w.r.t. 12, 24, and 48 regional branches). Here we generate $\pi_c^m$ from range $[0.1,0.9]$ for all the U sets and checked that the generated class priors are not all identical.
% As this dataset is naturally in a Non-IID pattern, so we do not impose class-prior shift.
% For model training, we use the cross-entropy loss and Adam \citep{kingma2014adam} optimizer with a learning rate of $1e-4$ and train 100 rounds. We use ResNet18 \citep{he2016deep} as backbone for experiments.

\newpage
\section{More Experimental Results on the Benchmark Datasets}
\label{app:more}

\subsection{Detailed Statistics of Figure \ref{fig:mnist_ablation_a}}

We show detailed statistics of Figure \ref{fig:mnist_ablation_a} in Table \ref{tb:noise_robustness}. With different noisy class priors, even with challenging $\epsilon=0.8$ and $\epsilon=1.6$, our method still achieves low error rate, which verify the robustness and effectiveness of our method.

\begin{table}[h]
\vspace{-3mm}
\renewcommand\arraystretch{1.1}
\centering
\caption{Inaccurate class priors experiments with different noise ratio $\epsilon$ on MNIST under Non-IID setting with 5 clients and 10 sets for every client (mean error (std)).}
\label{tb:noise_robustness}
\scalebox{0.95}{
\begin{tabular}{c|cccc}
\toprule
$\epsilon=0$ (Clean)&$\epsilon=0.2$&$\epsilon=0.4$&$\epsilon=0.8$&$\epsilon=1.6$\\
\hline
2.98 (1.72) & 3.02 (1.30) & 3.10 (0.96) & 3.02 (1.36) & 3.49 (1.74)
\\
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\end{table}

\subsection{Detailed Statistics of Figure \ref{fig:mnist_ablation_b}}
We show detailed statistics of Figure \ref{fig:mnist_ablation_b} in Table \ref{tb:accessible_data}. With more Non-IID data, our method performs better, which validates that more unlabeled Non-IID data can be helpful for FL.

\begin{table}[ht]
\vspace{-3mm}
\renewcommand\arraystretch{1.1}
\centering
\caption{Experiments on accessible data amount under the Non-IID setting  (mean error (std)).}
\label{tb:accessible_data}
\scalebox{0.95}{
\begin{tabular}{ccccc}
\toprule
5k & 10k & 15k & 20k & 25k\\
\hline
3.56 (0.09) & 2.62 (0.07) & 1.97 (0.38) & 1.75 (0.11) & 1.72 (0.13)
\\
\bottomrule
\end{tabular}
}
\end{table}

\subsection{Different Combinations of $E$ and $B$}
We compare our method with different combinations of $E$ and $B$ on benchmark dataset MNIST in the Non-IID setting. The classification error rate (mean and std) is consistently small as presented (cf. Table \ref{tb:mnist_eb}), which indicates our method can work under a wide range combinations of $E$ and $B$.
\begin{table}[h]
%\vspace{-5mm}
\renewcommand\arraystretch{1.1}
\centering
\caption{Experiments using different combinations of training batch size $B$ and local update epoch $E$ on benchmark dataset MNIST in the Non-IID setting (mean error (std)).}
\label{tb:mnist_eb}
\scalebox{0.85}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
    \toprule
    E     & \multicolumn{3}{c|}{1} & \multicolumn{3}{c|}{4} & \multicolumn{3}{c}{16} \\
    \hline
    B     & 16    & 128   & $\infty$ & 16    & 128   & $\infty$ & 16    & 128   & $\infty$ \\
    \hline
    %\multicolumn{1}{c|}{Error} 
    Error & \begin{tabular}[c]{@{}c@{}}7.99\\ (9.83) \end{tabular}  & \begin{tabular}[c]{@{}c@{}}2,93\\ (1.20) \end{tabular} & \begin{tabular}[c]{@{}c@{}}3.69\\ (0.88) \end{tabular} & \begin{tabular}[c]{@{}c@{}}2.54\\ (1.09) \end{tabular} & \begin{tabular}[c]{@{}c@{}}4.16\\ (3.44) \end{tabular}  & \begin{tabular}[c]{@{}c@{}}2.81\\ (0.37) \end{tabular}  & \begin{tabular}[c]{@{}c@{}}2.92\\ (1.12) \end{tabular} &\begin{tabular}[c]{@{}c@{}}3.51 \\ (1.88) \end{tabular} & \begin{tabular}[c]{@{}c@{}}2.88\\ (1.06) \end{tabular} \\
   % & & & & & & & & & 
    \bottomrule
    \end{tabular}%
    }
\end{table}%



% \newpage
\subsection{Benchmark Experiments on Clients with Different Sets}

Here we conduct experiments on benchmark datasets under IID and Non-IID setting with 5 clients and different sets for each client (10, 20, 30, 40, 50). The experimental results are shown in Table \ref{tb:clinets_with_diff_sets}, which further indicates the effectiveness of our method even under this challenging setting.


\begin{table}[h]
\renewcommand\arraystretch{1.1}
  \centering
\caption{Quantitative comparison of our method with the baseline methods on benchmark datasets under Non-IID and IID setting (mean error (std)) with different sets for each client. The best method (paired t-test at significance level 5\%) is highlighted in boldface.} 
\label{tb:clinets_with_diff_sets}
\scalebox{0.88}{
    \begin{tabular}{c|c|c|c|c|c}
    \toprule
    \multicolumn{6}{l}{\textbf{IID Task with 5 Clients}} \\
    \hline
    \hline
    Dataset  & \multicolumn{1}{c}{FedPL} & \multicolumn{1}{c}{FedLLP} & FedLLP-VAT & FedUL & FedAvg 10\% \\
    \hline
    MNIST    & 3.74 (0.78) & 5.22 (5.38) & 2.24 (0.05) & \textbf{1.19 (0.11)} & 2.21 (0.07) \\
    \hline
    CIFAR10    & 45.49 (2.74) & 84.16 (0.71) & 86.01 (2.54) & \textbf{31.17 (2.80)} & 42.27 (1.06) \\
    \hline
    \multicolumn{6}{l}{\textbf{Non-IID Task with 5 Clients}} \\
    \hline
    \hline
    Dataset  & \multicolumn{1}{c}{FedPL} & \multicolumn{1}{c}{FedLLP} & FedLLP-VAT & FedUL & FedAvg 10\% \\
    \hline
    MNIST    & 12.03 (2.89) & 4.26 (3.20) & 3.88 (2.89) & \textbf{2.31 (1.14)} & 3.42 (0.20) \\
    \hline
    CIFAR10    & 59.06 (3.73) & 62.44 (16.99) & 59.72 (18.73) & \textbf{35.46 (1.40)} & 53.13 (0.22) \\

    \bottomrule
    \end{tabular}}%
\end{table}%



% \newpage
\subsection{Benchmark Experiments with More Clients}
To study the influence of the number of clients, here we further conduct benchmark experiments on both MNIST and CIFAR10 with 10 clients. The detailed results are shown in Table \ref{tb:comp_sota_10clients}. The observations are similar to Table \ref{tb:comp_sota}. 
% Further, we show the empirical training loss curves and validation error curves in Figure \ref{fig:training_curve}, we find that our proposed method FedUL converges quickly and achieves much lower validation error.

\begin{table}[h]
\renewcommand\arraystretch{1.1}
\centering
\caption{Quantitative comparison of our method with the baseline methods on benchmark datasets under Non-IID and IID setting (mean error (std)). The best method (paired t-test at significance level 5\%) is highlighted in boldface.} 
% \Xiaoxiao{Pls add explanation for `Avg\%' :)}
\label{tb:comp_sota_10clients}
\scalebox{0.88}{
    \begin{tabular}{c|c|ccc|c|c}
    \toprule
    \multicolumn{7}{l}{\textbf{IID Task with 10 Clients}} \\
    \hline
    \hline
    Dataset & Sets  & FedPL & FedLLP & FedLLP-VAT & FedUL & FedAvg 10\% \\
    \hline
    \multirow{3}[2]{*}{MNIST} & 10    & 2.19 (0.04) & 10.11 (7.12) & 25.83 (22.64) & \textbf{0.74 (0.14)} & \multirow{3}[2]{*}{1.58 (0.23)} \\
          & 20    & 2.55 (0.30) & 24.23 (17.52) & 28.40 (23.20) & \textbf{1.05 (0.05)} &  \\
          & 40    & 3.13 (0.25) & 32.53 (16.93) & 34.46 (15.46) & \textbf{1.47 (0.11)} &  \\
    \hline
    \multirow{3}[2]{*}{CIFAR10} & 10    & 40.47 (0.58) & 76.23 (1.47) & 76.25 (1.65) & \textbf{20.40 (0.63)} & \multirow{3}[2]{*}{33.57 (1.03)} \\
          & 20    & 46.44 (0.71) & 78.10 (3.58) & 76.26 (3.83) & \textbf{21.61 (0.23)} &  \\
          & 40    & 51.58 (1.18) & 79.10 (2.34) & 80.44 (1.60) & \textbf{22.71 (0.17)} &  \\
    \hline
    \multicolumn{7}{l}{\textbf{Non-IID Task with 10 Clients}} \\
    \hline
    \hline
    Dataset & Sets  & FedPL & FedLLP & FedLLP-VAT & FedUL & FedAvg 10\% \\
    \hline
    \multirow{3}[2]{*}{MNIST} & 10    & 12.24 (1.36) & 20.81 (14.72) & 17.26 (10.39) & \textbf{1.91 (0.16)} & \multirow{3}[2]{*}{3.03 (0.24)} \\
          & 20    & 5.73 (0.89) & 17.67 (11.48) & 18.45 (4.30) & \textbf{1.45 (0.27)} &  \\
          & 40    & 4.16 (0.56) & 14.98 (10.11) & 13.62 (5.47) & \textbf{1.27 (0.12)} &  \\
    \hline
    \multirow{3}[2]{*}{CIFAR10} & 10    & 68.53 (1.14) & 84.11 (2.63) & 82.17 (2.58) & \textbf{39.20 (0.79)} & \multirow{3}[2]{*}{52.48 (1.55)} \\
          & 20    & 61.49 (1.42) & 71.69 (7.59) & 72.34 (7.39) & \textbf{34.12 (0.57)} &  \\
          & 40    & 55.89 (2.19) & 58.21 (4.95) & 59.42 (9.59) & \textbf{32.21 (1.02)} &  \\
    \bottomrule
    \end{tabular}}%
    % \vspace{-5mm}
\end{table}%


% \begin{figure}[t]
% \vspace{-1mm}
% \centering
% \includegraphics[width=\textwidth]{paper/figures/training_curve.pdf}
% \vspace{-3mm}
% \centering
% \caption{Training curves of learning from 10, 20 and 50 U sets within a FL system with 10 clients. Dashed curves are the empirical training losses and solid curves are the validation errors (in percentage). Dark colors show the mean errors (losses) of 3 trials and light colors show the standard deviations.}
% \label{fig:training_curve}
% \vspace{-3mm}
% \end{figure}







==> Federated Learning with Only Unlabeled Datasets final/sections/intro.tex <==
\section{Introduction}
\label{sec:intro}
\emph{Federated learning} (FL) has received significant attention from both academic and industrial perspectives
% since it can bring separate data sources together and build machine learning models in a collaborative but private manner.
in that it can bring together separate data sources
and allow multiple clients to train a central model in a collaborative but private manner \citep{mcmahan2017communication,kairouz2019advances,yang2019federated}.
So far, the majority of FL researches focused on the \emph{supervised} setting, requiring collected data at each client to be \emph{fully labeled}.
In practice, this may hinder the applicability of FL since manually labeling large-scale training data can be extremely costly, and sometimes may not even be possible for privacy concerns in for example medical diagnosis \citep{ng2021federated}.

% 1. the more data, the better
% 2. labeling cost--unlabeled
% 3. privacy
% 4. client drift
% 5. easy to implement, no additional computational cost

To promote the applicability of FL, we are interested in a challenging \emph{unsupervised FL} setting where \emph{only unlabeled}~(U) data are available at the clients under the condition described blow.
Our goal is still to train a classification model that can predict accurate class labels.
% in the FL setup.
% The problem is extremely difficult since without any labels, the clients cannot compute their local gradients and the central server cannot update its model based on them.
It is often observed that the clients collect their own data 
% at different time points or from different geographic locations, 
with different temporal and/or spatial patterns,
e.g., a hospital (data center) may store patient data every month or a particular user (mobile device) may take photos at different places.
Therefore,
we consider a realistic setting that the U data at a client come in the form of \emph{separate data sets}, and the data distribution of each U set and the number of U sets available at each client may \emph{vary}.
Without \emph{any} labels, it is unclear whether FL can be performed effectively.
% FL becomes significantly harder than before.
% since it is unclear how to compute the local gradients at each client and how to aggregate them for updating the global model.

In this paper, we show the possibility:
% that 
the aforementioned unsupervised FL problem can be solved 
if the class-prior probabilities are shifted while the class-conditional distributions are shared between the available U sets at the clients,
and these class priors are known to the clients.
% We do not require \emph{any} labels to be known, only assume the class priors within each of the involved data sets are available.
Such a learning scenario is conceivable in many real-world problems.
For example, the hospital may not release the diagnostic labels of patients
% patients' diagnostic labels 
due to privacy concerns, but the morbidity rates of diseases (corresponding to the class priors) may change over time and can be accessible from public medical reports \citep{croft2018urban};
moreover, in many cases it is possible to estimate the class priors much more cheaply
% than the ground-truth labels 
than to collect ground-truth labels \citep{quadrianto09jmlr,book:Sugiyama+etal:2022}.

Based on this finding, we propose the \emph{federation of unsupervised learning}~(FedUL) (see Figure~\ref{fig:framework}).
In FedUL,
% where 
the original clients with U data are transformed to surrogate clients with (surrogate) labeled data and then supervised FL can be applied, which we call the surrogate task.
% and then the underlying model can be recovered through certain transition functions.
Here, the difficulty is how to infer the wanted model for the original classification task from the model learned by the surrogate task.
We solve this problem by bridging the original and surrogate class-posterior probabilities with certain injective transition functions.
% Then we implement it 
This can be implemented by adding a specifically designed transition layer to the output of each client model, so that the learned model is guaranteed to be a good approximation of the original class-posterior probability.

\begin{figure}[t]
\vspace{-.4cm}
{\centering
\includegraphics[width=\textwidth]{figures/fig1.pdf}}
% \vspace{-.1cm}
{\footnotesize
In the left panel, each client $\fc$ ($c\in[C]$) has access to \emph{fully labeled data}, and a global model $\boldf$ can be trained using a supervised FL scheme, e.g., Federated Averaging (FedAvg) \citep{mcmahan2017communication}.
In the right panel, each client has access to only unlabeled~(U) data coming in the form of separate sets, where supervised FL methods cannot be directly applied.
We propose FedUL that treats the indexes of the U sets as \emph{surrogate labels},
transforms the local U datasets to (surrogate) labeled datasets,
and formulates a surrogate supervised FL task.
Then we modify each client model to be compatible with the surrogate task by adding a fixed transition layer $\bQ_c$ to the original model output $\fc$.
% (which yields $\gc$).
FedUL can incorporate existing supervised FL methods as its base method for surrogate training, and the wanted model $\boldf$ can be retrieved from the surrogate model.
}
\vspace{-.2cm}
\caption{Illustration of standard supervised FL scheme vs. proposed FedUL scheme.
% for a 3-class classification problem.
}
\label{fig:framework}
\vspace{-.3cm}
\end{figure}

FedUL has many key advantages.
On the one hand, FedUL is a very general and flexible solution: it works as a wrapper that transforms the original clients to the surrogate ones and therefore is compatible with many supervised FL methods, e.g., FedAvg.
% and adds no additional communication cost.
On the other hand,
FedUL is computationally efficient and easy-to-implement: 
since the added transformation layer is fixed and determined by the class priors, FedUL adds no more burden on hyper-parameter tuning and/or optimization.
Our contributions are summarized as follows:
\begin{itemize}[leftmargin=1em, itemsep=1pt, topsep=1pt, parsep=1pt]
    \item Methodologically, we propose a novel FedUL method that solves a certain unsupervised FL problem, expanding the applicability of FL.
    % providing new possibilities for FL.
    % employs a surrogate FL task, providing new perspectives for dealing with U data in FL.
    % Our algorithm is easy to implement and adds no additional communication cost. 
    \item Theoretically, we prove the optimal global model learned by FedUL from only U data converges to the optimal global model learned by supervised FL from labeled data under mild conditions.
    \item Empirically, we demonstrate the effectiveness of FedUL on benchmark and real-world datasets.
    % We also provide an ablation study of FedUL that analyzes its robustness against noisy class priors, different client numbers, local updating epochs and batch sizes.
\end{itemize}
% Our method provides new perspectives for solving unsupervised FL, and is suitable to be applied in practice given the theoretical and practical advantages.

% \Nan{The last two paragraphs need to be modified after modifying the whole paper.}\\
% \Xiaoxiao{Shall we also mention 'easy to implement in practice' and no additional communication cost in our contributions? no communication cost}\\
% %\Xiaoxiao{We may want to add short related work and roadmap here.}

\textbf{Related Work:}
% \textit{FL} is an emerging paradigm in distributed machine learning, which allows different clients to collaboratively train models together without data sharing.
FL has been extensively studied in the supervised setting.
One of the most popular supervised FL paradigms is FedAvg~\citep{mcmahan2017communication} which aggregates the local updates at the server and transmits the averaged model back to local clients.
In contrast, FL in the unsupervised setting is less explored.
Recent studies have shown the possibility of federated clustering with U data~\citep{ghosh2020efficient,pmlr-v139-dennis21a}.
% However, these clustering based methods are sub-optimal for classification goals since they rely on geometric or information-theoretic assumptions to build their learning objectives \citep{chapelle06SSL}, which may not hold in practice.
However, these clustering based methods rely on geometric or information-theoretic assumptions to build their learning objectives \citep{chapelle06SSL}, and are suboptimal for classification goals.
Our work is intrinsically different from them in the sense that we show the possibility of federated classification with U data based on \emph{empirical risk minimization}~(ERM) \citep{vapnik98SLT}, and therefore the optimal model recovery can be guaranteed.

Learning from multiple U sets has also been studied in classical centralized learning.
Mainstream methods include \emph{learning with label proportions}~(LLP) \citep{quadrianto2009estimating} and \emph{U$^m$ classification}~\citep{lu2021binary}. 
The former learns a multiclass classifier from multiple U sets based on \emph{empirical proportion risk minimization}~(EPRM)~\citep{yu2014learning},
while the latter learns a binary classifier from multiple U sets based on ERM.
EPRM is inferior to ERM since its learning is not consistent.
Yet, it is still unexplored how to learn a multiclass classification model from multiple U sets based on ERM.
% To the best of our knowledge, we are the first to tackle this problem in the FL setup, where our method can be seen as a generalization of U$^m$
% classification to the multi-class FL setup.
To the best of our knowledge, this work is the first attempt to tackle this problem in the FL setup, which is built upon the binary U$^m$ classification in centralized learning.
A full discussion of related work can be found at Appendix~\ref{sec:related}.

% Our problem setting in the centralized setup is more related to LLP which learns a multi-class classification model from multiple U datasets with known class priors, rather than UU which learns only binary classification models.
% Our method in the centralized setup is more related to UU which is based on ERM, rather than LLP which is based on \emph{proportion risk minimization}~\citep{yu2014learning}.


% \iffalse
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{paper/figures/fig1.pdf}
%     \caption{Comparison of our setting and proposed method vs FedAvg.}
%     \label{fig:framework}
% \end{figure}
% \fi





==> Federated Learning with Only Unlabeled Datasets final/sections/method.tex <==
% \section{Problem Setup}
% \label{sec:setup}
\section{Standard Federated Learning}
\label{sec:fed}
We begin by reviewing the standard FL.
% of a classification model.
Let us consider a $K$-class classification problem with the feature space $\mathcal{X}\subset\R^d$ and the label space $\mathcal{Y}=[K]$, where $d$ is the input dimension and $[K]\coloneqq\{1,\ldots,K\}$.
Let $\bx \in \mathcal{X}$ and $y \in \mathcal{Y}$ be the input and output random variables following an underlying joint distribution with density $p(\bx,y)$, which can be identified via the class priors $\{\pi^k= p(y=k)\}_{k=1}^K$ and the class-conditional densities 
% $\{P^k\coloneqq p(\bx\mid y=k)\}_{k=1}^K$.
$\{p(\bx\mid y=k)\}_{k=1}^K$.
Let $\boldf:\mathcal{X}\to\R^K$ be a classification model that assigns a score to each of the $K$ classes for a given input $\bx$ and then outputs the predicted label by $y_{\rm{pred}} = \mathop{\argmax}_{k\in [K]}(\boldf(\bx))_k$, where $(\boldf(\bx))_k$ is the $k$-th element of $\boldf(\bx)$. 
% and can be interpreted as the relevance of the $k$-th class for the input $\bx$.
% Typically, we consider the following embedding based form of $f$:
% \begin{align*}
%     f(\bx)=W\cdot \phi_\btheta(\bx),
% \end{align*}
% where $\phi_\btheta:\mathcal{X}\to\R^b$ (parameterized by $\btheta$) maps the input $\bx$ to a $b$-dimensional embedding, and $W\in\R^{K\times b}$ uses this embedding to produce the scores, a.k.a. logits,\Xiaoxiao{logits by definition include normalization} for the $K$ classes as $W\cdot \phi_\btheta(\bx)$.

In the standard FL setup with $C$ clients,
for $c\in[C]$,
the $c$-th client
% each client $c\in[C]$ 
has access to a labeled training set
$\mathcal{D}_c = \{(\bx^c_i,y^c_i)\}_{i=1}^{n_c}{\sim}p_c(\bx,y)$ of sample size $n_c$
% $\mathcal{D}_c = \{(\bx^c_i,y^c_i)\}_{i=1}^{n_c}$ of sample size $n_c$ independent and identically distributed~(IID) \Xiaoxiao{Do we have to put the IID condition here?} according to an underlying local data distribution $p_c(\bx,y)$, 
% i.e., $(\bx^c_i,y^c_i)\sim p_c(\bx,y)$,
and learns its local model $\fc$ by minimizing the risk
% \Xiaoxiao{Maybe we should use normal `risk' to reduce attention?} 
% defined as follows:
\begin{align} 
\label{eq:risk}%
    R_c(\fc)\coloneqq\mathbb{E}_{(\bx,y)\sim p_c(\bx,y)}[\ell(\fc(\bx),y)].
\end{align}
Here, $\mathbb{E}$ denotes the expectation,
$\ell:\mathbb{R}^K\times\mathcal{Y}\to\mathbb{R}_{+}$ is a proper loss function, e.g., the \emph{softmax cross-entropy loss} $\ell_{\rm{ce}}(\fc(\bx),y)=-\sum\nolimits_{k=1}^K\boldsymbol{1}(y=k)\log\left(\frac{\exp((\fc(\bx))_{k})}{\sum\nolimits_{i=1}^K\exp((\fc(\bx))_{i})}\right)=\log\left(\sum\nolimits_{i=1}^K\exp((\fc(\bx))_{i})\right)-(\fc(\bx))_{y}$,
where $\boldsymbol{1}(\cdot)$ is the indicator function.
In practice, ERM is commonly used to compute an approximation of $R_c(\fc)$ based on the client's local data $\mathcal{D}_c$ by $\hat{R}_c(\fc;\mathcal{D}_c)=\frac{1}{n_c}\sum\nolimits_{i=1}^{n_c}\ell(\fc(\bx^c_i),y^c_i)$. 
% \Xiaoxiao{Totally makes sense to me!}
% \begin{align}
% \label{eq:emp-risk}%
% \hat{R}_c(\boldf;\mathcal{D}_c)\coloneqq\frac{1}{n_c}\sum\nolimits_{i=1}^{n_c}\ell(\boldf(\bx^c_i),y^c_i).
% \end{align}
% an empirical estimate of the classification risk based on $\mathcal{D}_c$:
% \begin{align}
% \label{eq:risk}%
% \fc = \argmin_{\boldf\in\mathcal{F}}\hat{R}(\boldf;\mathcal{D}_c):=\frac{1}{n_c}\sum\nolimits_{i=1}^{n_c}\ell(\boldf(\bx^c_i),y^c_i),
% \end{align}
% where $\mathcal{F}=\{\boldf:\mathcal{X}\to\R^K\}$ is a class of measurable functions.

The goal of standard FL~\citep{mcmahan2017communication} is that the $C$ clients collaboratively train a global classification model $\boldf$
that generalizes well with respect to $p(\bx,y)$,
% by minimizing
% $R(\boldf)=\frac{1}{C}\sum\nolimits_{c=1}^C R_c(\boldf)$
% , the $C$ clients are interested in collaboratively training a global classification model $\fs$ that generalizes well with respect to $p(\bx,y)$, without sharing their local data $\mathcal{D}_c$.
% that generalizes well with respect to $p(\bx,y)$,
without sharing their local data $\mathcal{D}_c$.
The problem can be formalized as minimizing the aggregated risk:
\begin{align}
\label{eq:supervised-FL}%
    R(\boldf)=\frac{1}{C}\sum\nolimits_{c=1}^C R_c(\boldf).
\end{align}
% $R(\boldf)\coloneqq\frac{1}{C}\sum\nolimits_{c=1}^C R_c(\boldf)$.
% \Xiaoxiao{If we do not have enough space, I think we can move this paragraph to appendix.}
Typically, we employ a server to coordinate the iterative distributed training as follows:
% Typically, we wish to minimize the aggregated risk
% $R(\boldf)=\frac{1}{C}\sum\nolimits_{c=1}^C R_c(\boldf)$.
% In practice, we employ a server to coordinate the iterative distributed training as follows:
% then the server facilitates the joint iterative distributed training as follows:
\begin{itemize}[leftmargin=1em, itemsep=1pt, topsep=1pt, parsep=1pt]
    \item in each global round of training, the server broadcasts its current model $\fs$ to all the clients $\{\fc\}_{c=1}^C$;
    \item each client $c$ copies the current server model $\fc=\fs$, performs $L$ local step updates
    % based on its empirical estimate of the classification risk:
    \begin{align}
    \label{eq:client-update}%
        \fc\leftarrow\fc-\alpha_l\cdot\nabla\hat{R}_c(\fc;\mathcal{D}_c),
    \end{align}
    % $\fc\leftarrow\fc-\alpha_l\cdot\nabla\hat{R}_c(\fc;\mathcal{D}_c)$,
    where $\alpha_l$ is the local step-size, and sends $\fc-\fs$ back to the server;
    \item the server aggregates the updates $\{\fc-\fs\}_{c=1}^C$ to form a new server model using FedAvg:
    % $\fs\leftarrow\fs-\alpha_g\cdot\sum\nolimits_{c=1}^C(\fc-\fs)$,
    % the server receives the updates from all clients $\{\fc-\fs\}_{c=1}^C$ and aggregates them to form the new server model using \emph{Federated Averaging} (FedAvg) \citep{mcmahan2017communication}:
    \begin{align}
    \label{eq:server-update}%
        \fs\leftarrow\fs-\alpha_g\cdot\sum\nolimits_{c=1}^C(\fc-\fs),
    \end{align}
    where $\alpha_g$ is the global step-size.
\end{itemize}

% %simplified
% If the local data distributions satisfy $\forall c, p_c(\bx,y)=p(\bx,y)$, a good generalization of the standard FedAvg scheme is guaranteed~\citep{li2019convergence,hlsy21}.
% % This is the IID assumption made by many distributed optimization algorithms.
% However, since the clients independently collect their own training data which may vary significantly, such a strict independent and identically distributed~(IID) data assumption rarely holds,
% causing training difficulties
% and performance degradation of the FL models~\citep{zhao2018federated,li2019convergence, li2021fedbn}.


% \Nan{As data can be non-IID in many ways, in this paper, we refer to the situation when different clients $p_{c_1}(\bx,y)\neq p_{c_2}(\bx,y)$ for different clients $c_1$ and $c_2$} \Xiaoxiao{I think this is the default definition. Otherwise, ppl may discuss whether it's $p(x)$ or $p(y)$ or $p(x|y)$}

% \Nan{Discuss non-IID, the relationship between $p_c$ and $p$.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Federated Learning with Only Unlabeled Datasets}
\section{Federated Learning: No Label No Cry}
\label{sec:fed-u}
Next, we formulate the problem setting of FL with only U training sets, propose our method called \emph{federation of unsupervised learning}~(FedUL), and provide the theoretical analysis of FedUL.
All proofs are given in Appendix~\ref{sec:proof}.
% \Xiaoxiao{This section is very clear to me :)}

% \subsection{Motivation}
% \textcolor{red}{Standard FL converges...but when data are non-iid, the performance drops.}

\subsection{Problem Formulation}
\label{sec:formulate}
% \Xiaoxiao{Nan: let us use `FL' for federated learning, and `FedAvg' for federated averaging.}
% In this paper, we consider a challenging setting of FL with only \emph{unlabeled} datasets.
% In contrast to standard FL where each client has access to the fully labeled training data, for each client $c\in[C]$, we are given only $m$ $(m\geq K)$ sets of unlabeled samples $\mathcal{U}_{c}=\{\mathcal{U}_{c}^{j}\}_{j=1}^{m}$, where $\mathcal{U}_{c}^{j} = \{\bx_{1}^{c,j},\ldots, \bx_{n_{c,j}}^{c,j}\}$
% and $n_{c,j}$ denotes the sample size of the $j$-th U set.
% Each U set can be seen as drawn from a mixture of the original class-conditional densities, i.e.,
% % $m$ marginal densities $\{p_c^{j}(\bx)\}_{j=1}^{m}$, where:
% \begin{align}
% \mathcal{U}_{c}^{j}\sim p_c^{j}(\bx)=\sum\nolimits_{k=1}^K\pi_{c,k}^j p(\bx\mid y=k),
% \label{ptr}
% \end{align}
% \sloppy
% where $\pi_{c,k}^j=p_{c}^{j}(y = k)$ denotes the $k$-th class prior of the $j$-th U set, and these class priors form a full column rank matrix $\bpi_c\in\R^{m\times K}$ with the constraint that each row sums up to 1.


% In this paper, we consider a challenging setting where for each client $c\in[C]$,
% instead of fully labeled training data, we are given $\mc$ $(\mc\geq K)$ sets of \emph{unlabeled} samples $\mathcal{U}_{c}=\{\mathcal{U}_{c}^{m}\}_{m=1}^{\mc}$,
% where 
% % $\mathcal{U}_{c}^{m} = \{\bx_{1}^{c,m},\ldots, \bx_{n_{c,m}}^{c,m}\}$
% $\mathcal{U}_{c}^{m} = \{\bx_{i}^{c,m}\}_{i=1}^{n_{c,m}}$
% and $n_{c,m}$ denotes the sample size of the $m$-th  U set for client $c$.
In this paper, we consider a challenging setting: 
instead of fully labeled training data, each client $c\in[C]$ observes $\mc$ $(\mc\geq K, \forall c)$%
\footnote{Note that we do not require each client has the same number of U sets.
% the number of given U sets at each client is equal.
% , i.e. $ M_c=M, \forall c$.
We only assume the condition $\mc\geq K, \forall c$ to ensure the full column rank matrix $\Pi_c$, which is essential for FL with U training sets.}
sets of \emph{unlabeled} samples,  $\mathcal{U}_{c}=\{\mathcal{U}_{c}^{m}\}_{m=1}^{\mc}$,
where 
% $\mathcal{U}_{c}^{m} = \{\bx_{1}^{c,m},\ldots, \bx_{n_{c,m}}^{c,m}\}$
$\mathcal{U}_{c}^{m} = \{\bx_{i}^{c,m}\}_{i=1}^{n_{c,m}}$ denotes the collection of the $m$-th  U set for client $c$ 
with sample size $n_{c,m}$.
Each U set can be seen as a set of data points drawn from a mixture of the original class-conditional densities:
% $m$ marginal densities $\{p_c^{j}(\bx)\}_{j=1}^{m}$, where:
\begin{align}
\mathcal{U}_{c}^{m}\sim p_c^{m}(\bx)=\sum\nolimits_{k=1}^K\pi_{c}^{m,k}
p(\bx\mid y=k),
\label{ptr}
\end{align}
\sloppy
where $\pi_{c}^{m,k}=p_{c}^{m}(y = k)$ denotes the $k$-th class prior of the $m$-th U set at client $c$.
These class priors form a full column rank matrix $\Pi_c\in\R^{\mc\times K}$ with the constraint that each row sums up to 1.
Note that we do not require \emph{any} labels to be known, only assume the class priors within each of the involved datasets are available,
i.e., the training class priors $\pi_{c}^{m,k}$ and the test class prior $\pi^k=p(y=k)$.
% We call this problem \emph{FL with only unlabeled datasets}.
% \Nan{We do not assume the number of U sets are the same at each client}

% The assumption is reasonable in many real-world problems, in our hospital example, the hospitals may not release the patients' diagnostic labels due to privacy reasons, but the morbidity rates of diseases (corresponds to the class priors of diseases) can be accessible from related public medical reports \citep{croft2018urban}.%
% \footnote{See more examples on sentiment analysis in \citet{ardehaly2017mining}, semantic segmentation in \citet{tokunaga2020negative}, politics, e-commerce, and spam filtering in \citet{quadrianto09jmlr}.}

% \Nan{If we have space, introduce inter-U-set shift, inter-client shift, realistic IID assumption with training-test shift.}

% {\color{red} To make the problem mathematically solvable, among the $m$ sets of unlabeled data, we assume at least $K$ of them are different, i.e., $\exists j, j' \in \{1,\ldots,m\}$ such that $j \neq j' $ and $\pi_j \neq \pi_{j'}$.}

Our goal is the same as standard FL:
the $C$ clients are interested in collaboratively training a global classification model $\boldf$ that generalizes well with respect to $p(\bx,y)$,
but using only U training sets \eqref{ptr} on each local client.
% to obtain a classifier that generalizes well with respect to $\mathcal{D}$, despite the fact that it is unobserved.

% \begin{wraptable}{r}{0.45\textwidth}
% \begin{figure}[t]
% \centering
% \subfigure[]{
% \includegraphics[width=0.97\textwidth]{figures/graphical.pdf}
% }%
% \caption{Graphical model of
% }
% \label{fig:graphical}
% \end{figure}
% \end{wraptable}

\subsection{Proposed Method}
\label{sec:method}

%\Xiaoxiao{Nan: Do we need $M$ to be the same across clients? If not, we need to highlight it somewhere. Because in the experiment part, we use all equal $M$, which may mislead readers.}

As discussed, FedAvg is a representative approach for aggregating clients in the FL framework.
It also serves as the basis for many advanced federated aggregation techniques, e.g., Fedprox~\citep{li2018federated}, FedNova~\citep{wang2020tackling}, and SCAFFOLD~\citep{ karimireddy2020scaffold}.
However, these methods cannot handle clients \emph{without} labels.
% any labeled data, 
% which are necessary for them to compute local gradients.
% \Xiaoxiao{Not sure if this statement is too strong, I'll double check.}
To tackle
% solve 
this problem, we consider the construction of 
% \emph{surrogate clients} 
\emph{surrogate clients} 
by transforming the local U datasets into labeled datasets and modifying the local model such that 
% they are able to utilize the transformed datasets for local updates.
it is compatible with the transformed data for training.
% , and then we propose federated averaging with these surrogate clients.
% As such, our desired classification model can be identified from useful updates.

\paragraph{Local Data Transformation}
First, we transform the data for the clients.
For each client $c\in[C]$,
let $\overline{y}$ be the index of given U sets,
% By treating $\overline{y}$ as a surrogate label, 
% we first formulate the surrogate set classification task as a standard $m$-class classification problem.
and $\overline{p}_c(\bx,\overline{y})$ be an underlying joint distribution for the random variables $\bx\in \mathcal{X}$ and $\overline{y}\in [M]$, where $M=\max_{c\in[C]}M_c$.\footnote{To make the problem well-defined, for client $c$ with $\mc < M$, we set $\mathcal{U}_{c}^{m}=\emptyset$, $\forall M_c < m \leq M$.
% we set $\overline{\pi}^m_c=\epsilon$ where $\epsilon$ is a small positive number.
}
% For each client $c\in[C]$,
By treating $\overline{y}$ as a \emph{surrogate label}, 
% at each client, 
we may transform the original U training sets $\mathcal{U}_{c}=\{\mathcal{U}_{c}^{m}\}_{m=1}^{\mc}$ 
% designed for $K$-class classification 
to a labeled training set
for client $c$,
\begin{align}
    \overline{\mathcal{U}}_{c}=\{\bx_i,\overline{y}_i\}_{i=1}^{n_c}\sim \overline{p}_c(\bx,\overline{y}),
    \label{surro-set}
\end{align}
where $n_c=\sum_{m=1}^{\mc} n_{c,m}$.
% $\overline{\mathcal{U}}_{c}=\{\bx_i,\overline{y}_i\}_{i=1}^{n_c}\sim \overline{p}_c(\bx,\overline{y})$.
% designed for $M$-class classification.
Obviously,
the surrogate class-conditional density $\overline{p}_c(\bx\mid\overline{y}=m)$ corresponds to $p_c^{m}(\bx)$ in \eqref{ptr}, for $m\in [\mc]$. If $\exists \mc < m\leq M$, we pad $\overline{p}_c(\bx\mid\overline{y}=m)=0$.
The surrogate class prior $\overline{\pi}^m_c=\overline{p}_c(\overline{y}=m)$ can be 
estimated by
$n_{c,m}/n_c$.%
% \footnote{To make the problem solvable, if $\mathcal{U}_{c}^{m}=\emptyset$, we set $\overline{\pi}^m_c=\epsilon$ where $\epsilon$ is a small positive number.}
% We do not require that the number of given U sets at each client $M_c$ are equal, i.e., $\forall c, M_c=M$.
% If $M_c$ differs, we can simply set $M=\max_{c\in[C]}M_c$, and $\mathcal{U}_{c}^{m}=\emptyset$ where $m={M_c,\cdots,M}$ for each client $c$.

% Let $\gc:\mathcal{X}\to\R^M$ be a classification model which predicts the surrogate label $\overline{y}$ for a given input $\bx$.
Based on the data transformation, we then formulate a \emph{surrogate supervised FL task}: the $C$ clients aim to collaboratively train a global classification model $\bg:\mathcal{X}\to\R^{M}$ that predicts the surrogate label $\overline{y}$ for the given input $\bx$, without sharing their local data $\overline{\mathcal{U}}_{c}$.
This task can be easily solved by standard supervised FL methods.
More specifically, we minimize
% $R(\bg)\coloneqq\frac{1}{C}R_c(\bg)$ 
\begin{align}
    J(\bg)=\frac{1}{C}\sum\nolimits_{c=1}^CJ_c(\bg)\coloneqq\mathbb{E}_{(\bx,\overline{y})\sim \overline{p}_c(\bx,\overline{y})}[\ell(\bg(\bx),\overline{y})]
 \label{surro-obj}   
\end{align}
by employing a server $\bg$ that iteratively broadcasts its model to all local clients $\{\gc\}_{c=1}^C$ and aggregates local updates from all clients using e.g., FedAvg.
The local and global update procedures exactly follow \eqref{eq:client-update} and \eqref{eq:server-update} in standard FL.

Now a natural question arises: 
can we \emph{infer} our desired model $\boldf$ from the surrogate model $\bg$?
To answer it, we study the relationship between the original and surrogate class-posterior probabilities.

\begin{theorem} 
\label{thm:transformation}%
For each client $c\in[C]$, let
$\overline{\boldeta}_c:\mathcal{X}\to\Delta_{M-1}$ and $\boldeta:\mathcal{X}\to\Delta_{K-1}$
% $\overline{\boldeta}_c$ and $\boldeta$
be the surrogate and original class-posterior probability functions,
where $(\overline{\boldeta}_c(\bx))_m=\overline{p}_c(\overline{y}=m\mid\bx)$ for $m\in[M]$, $(\boldeta(\bx))_k=p(y=k\mid\bx)$ for $k\in[K]$,
$\Delta_{M-1}$ and $\Delta_{K-1}$ are the $M$- and $K$-dimensional simplexes.
Let $\overline{\bpi}_c=[\overline{\pi}^1_c,\cdots,\overline{\pi}^{M}_c]^\top$ and $\bpi=[\pi^1,\cdots,\pi^K]^\top$ be vector forms of the surrogate and original class priors, and $\Pi_c\in\R^{M\times K}$ be the matrix form of $\pi_{c}^{m,k}$ defined in \eqref{ptr}.
% $k\in[K]$,
% and $m\in[M]$.
% $(\boldeta(\bx))_k=p(y=k\mid\bx)$ and $\overline{\eta}_c^m(\bx)=\overline{p}(\overline{y}=m\mid\bx)$, where $k\in[K]$ and $m\in[M]$, be the class-posterior probabilities of the original and surrogate classification problems, respectively.
% Assume that the test classes are uniformly distributed, we have
Then we have
\begin{align}
    \overline{\boldeta}_c(\bx)=\bQ_c(\boldeta(\bx);\bpi, \overline{\bpi}_c,\Pi_c),
\end{align}
where the unnormalized version of vector-valued function $\bQ_c$ is given by
% \begin{align}
%     \bQ=\frac{\overline{\bpi}_c\cdot \bpi_c\cdot\frac{\boldeta(\bx)}{\bpi}}{}
% \end{align}
\begin{align*}
    \widetilde\bQ_c(\boldeta(\bx);\bpi, \overline{\bpi}_c,\Pi_c) =  D_{\overline{\bpi}_c}\cdot \Pi_c \cdot D^{-1}_{\bpi} \cdot \boldeta(\bx).
\end{align*}
$D_\ba$ denotes the diagonal matrix with diagonal terms being vector $\ba$ and $\cdot$ denotes matrix multiplication. $\bQ_c$ is normalized by the sum of all entries, i.e., $(\bQ_c)_i = \frac{(\widetilde \bQ_c)_i}{\sum_j (\widetilde \bQ_c)_j}$.
% \begin{equation}
% \overline{\eta}_j(\bx)=Q_j(\eta_k(\bx)),\quad \forall j = 1,\ldots,m, and \quad \forall k = 1,\ldots,K,
% \label{qfunc}
% \end{equation}
% where
% \begin{equation} \nonumber
% Q_j(\eta_k(\bx))=\frac{\rho_j(\sum_{k=1}^K\pi_k^j\eta_k(X))}{\sum_{j=1}^m\rho_j(\sum_{k=1}^K\pi_k^j\eta_k(\bx))}.
% \end{equation}

% \begin{equation}
% \overline{\eta}_j(x)=Q_j(\eta(x)),\quad \forall j = 1,\ldots,m,
% \end{equation}
% where
% \begin{equation} \nonumber
% Q_j(\eta(x))=\displaystyle\frac{a_j\cdot\eta(x)+b_j}{c\cdot\eta(x)+d},
% \end{equation}
% $a_j = {\rho}_j(\pi_j-\pi_{\mathcal{D}})$, $b_j = {\rho}_j\pi_{\mathcal{D}}(1-\pi_j)$, $c = \sum_{j=1}^m{\rho}_j(\pi_j-\pi_{\mathcal{D}})$, and $d = \sum_{j=1}^m{\rho}_j\pi_{\mathcal{D}}(1-\pi_j)$.
\label{theorem1}
\end{theorem}

Note that $\bpi$, $\overline{\bpi}_c$, and $\Pi_c$ are all fixed, $\bQ_c$ is deterministic and can be identified with the knowledge of $\bpi$, $\Pi_c$, and an estimate of $\overline{\bpi}_c$.
In addition, we note that if $\mc < M$, the last $M - \mc$ entries of $\bQ_c$ are padded with zero by construction.
% , we can identify $\bQ_c$ accurately.
We further study the property of $\bQ_c$ in the following lemma.

\begin{lemma}
For each client $c\in[C]$,
the transition function $\bQ_c: (\mathcal{X}\to\Delta_{K-1})\to(\mathcal{X}\to\Delta_{M-1})$ defined in Theorem~\ref{theorem1} is an injective function.
\label{lemm:injective}
\end{lemma}
In this sense, the transition function $\bQ_c$ naturally bridges the class-posterior probability of our \emph{desired} task $\boldeta(\bx)$ 
% which is what we want, 
and that of the \emph{learnable} 
% class-posterior probabilities of the 
surrogate task $\overline{\boldeta}_c(\bx)$
% which is what we can estimate
% The former is what we want; the latter is what we can estimate
given only U training sets.
This motivates us to embed the estimation of $\boldeta(\bx)$ into the estimation of $\overline{\boldeta}_c(\bx)$ at the client side.
% with bridge between $\boldf$ and $\bg$ via $Q$

% \begin{center}
% \emph{Aggregating all $C$ clients with such surrogate learning scheme makes unsupervised FL possible}! 
% \end{center}

\begin{algorithm}[t]
    \caption{Federation of unsupervised learning~(FedUL)}
    \label{alg}

    \textbf{Server Input:}
    initial $\fs$, 
    global step-size $\alpha_g$,
    and global communication round $R$\\
    \textbf{Client $c$'s Input:}
    local model $\fc$, 
    unlabeled training sets $\mathcal{U}_{c}=\{\mathcal{U}_{c}^{m}\}_{m=1}^{\mc}$, 
    class priors $\Pi_c$ and $\bpi$,
    local step-size $\alpha_l$,
    and local updating iterations $L$
    \begin{algorithmic}[1]
    \State{We start with initializing clients with \textbf{Procedure A}.}
    \State {For $r = 1 \to R$ rounds, we run \textbf{Procedure B} and \textbf{Procedure C} iteratively .}
	\Procedure{\textbf{A}. ClientInit}{$c$} 
     \State transform $\mathcal{U}_{c}$ to a surrogate labeled dataset $\overline{\mathcal{U}}_{c}$ according to \eqref{surro-set}
     \State modify $\boldf$ to $\bg_c=\bQ_c(\boldf)$, where $\bQ_c$ is computed according to Theorem~\ref{theorem1}
    %  \STATE Let $\bg_c=\bQ_c(\boldf)$ and $\mathcal{A}_c$ be a SGD-like optimizer working on $\bg_c$
    \EndProcedure
    
    \Procedure{\textbf{B}. ClientUpdate}{$c$}
    \State{$\fc\leftarrow\fs$} \Comment{Receive updated model from \textsc{ServerExecute}}
    \State{$\bg_c \leftarrow \bQ_c(\fc)$}
    \For{$l=1\to L$}
                %       \State{fetch mini-batch $\overline{\mathcal{U}}_{mini}$ from $\overline{\mathcal{U}}_{c}$}
                %   \State { $\hat{J}_c(\bg_c;\overline{\mathcal{U}}_{mini})=\frac{1}{n_c}\sum\nolimits_{i=1}^{n_c}\ell(\bQ_c(\boldf(\bx_i)),\overline{y}_i)$} 
                  \State{ $\bg_c\leftarrow\bg_c-\alpha_l\cdot\nabla\hat{J}_c(\bg_c;\overline{\mathcal{U}}_{c})$}
                  \Comment{SGD update based on objective \eqref{surro-obj}}
                % \State{ $\fc\leftarrow\fc-\alpha_l\cdot\nabla\hat{J}_c(\fc;\overline{\mathcal{U}}_{c})$}
                %   \Comment{Updates on $\gc$ induces an update on $\boldf$}
                
                \State{ $\fc\leftarrow\fc-\alpha_l\cdot\nabla\hat{J}_c(\bQ_c(\fc);\overline{\mathcal{U}}_{c})$}
                %  \Comment{SGD updates based on objective \eqref{surro-obj-reformulate}}
                \Comment{The update on $\gc$ induces an update on $\fc$}
    \EndFor
    % \State{reduce xxxx to $\fc$ \Xiaoxiao{To Do}}
                  \State{send $\fc-\fs$ to \textsc{ServerExecute}}
    \EndProcedure{}
    \Procedure{\textbf{C}. ServerExecute}{$r$} 
        \State{receive local models' updates $\{\fc-\fs\}_{c=1}^C$ from \textsc{ClientUpdate}}
        \State{$\fs\leftarrow\fs-\alpha_g\cdot\sum\nolimits_{c=1}^C(\fc-\fs)$}
        \Comment{FL aggregation}
        \State{broadcast $\fs$ to \textsc{ClientUpdate}}
    \EndProcedure
    \end{algorithmic}
\end{algorithm}

\paragraph{Local Model Modification}
Second, we modify the model for the clients.
Let $\boldf(\bx)$ be the original global model output that estimates $\boldeta(\bx)$.
At each client $c\in[C]$, we implement $\bQ_c$ by adding a transition layer following $\fc$ and then we have $\bg_c(\bx)=\bQ_c(\fc(\bx))$.
Based on the local model modification, \eqref{surro-obj} can be reformulated as follows:
% $
% J(\boldf)
% =\frac{1}{C}\sum\nolimits_{c=1}^CJ_c(\bQ_c(\boldf))
% \coloneqq\mathbb{E}_{(\bx,\overline{y})\sim \overline{p}_c(\bx,\overline{y})}[\ell(\bQ_c(\boldf(\bx)),\overline{y})]$.
\begin{align}
\label{surro-obj-reformulate} 
% \hspace{-0.76cm}
J(\boldf)
=\frac{1}{C}\sum\nolimits_{c=1}^CJ_c(\bQ_c(\boldf))
\coloneqq\mathbb{E}_{(\bx,\overline{y})\sim \overline{p}_c(\bx,\overline{y})}[\ell(\bQ_c(\boldf(\bx)),\overline{y})].
% &=\mathbb{E}_{(\bx,\overline{y})\sim \overline{p}_c(\bx,\overline{y})}[\ell(\bg(\bx),\overline{y})]=J(\bg)=\frac{1}{C}\sum\nolimits_{c=1}^CJ_c(\bg).
 \end{align}
% \eqref{surro-obj-reformulate} can be estimated via ERM.

\vspace{-.15cm}
\begin{wrapfigure}{r}{0pt}
\includegraphics[width=0.33\textwidth]{figures/graphical.pdf}
\caption{
Graphical representation of supervised FL (in blue) and FedUL (in green).
\label{fig:graphical_mapping}}
\vspace{-.8cm}
\end{wrapfigure}
Therefore, local updates on the surrogate model $\bg_c$ naturally yield updates on the underlying model $\fs$.
Now we can aggregate the surrogate clients by a standard FL scheme.
A detailed algorithm, using FedAvg as an example, is given in Algorithm~\ref{alg}.


\paragraph{Remarks}
The relationship elucidating the supervised and surrogate FL paradigms (for a single client) is visually shown in Figure \ref{fig:graphical_mapping}.
The blue part illustrates a supervised FL scheme: 
the global model is $\boldf(\bx)$ parameterized by $\btheta$;
the loss is $R(\boldf;y)$ in \eqref{eq:supervised-FL} where labels $y$ are observed.
However, we cannot observe $y$ and thus employ a surrogate FedUL scheme which is shown in green:
% The green part illustrates a surrogate learning scheme with 
the global model is $\bg(\bx)$ directly modified from $\boldf$;
the loss is $J(\bg;\overline{y})$ in \eqref{surro-obj} where $\overline{y}$ are surrogate labels.

% \begin{center}
% \emph{Aggregating all the clients with such surrogate learning scheme makes unsupervised FL possible}! 
% \end{center}

\iffalse
\begin{algorithm}[t]
    \caption{Federated Averaging with Surrogate Clients}
    \label{alg}
    \begin{algorithmic}
    \STATE \textbf{Server Input:}
    initial $\fs$, 
    global step-size $\alpha_g$,
    and global commnunication round $R$
    \STATE \textbf{Client $c$'s Input:}
    local model $\fc$, 
    unlabeled training sets $\mathcal{U}_{c}=\{\mathcal{U}_{c}^{m}\}_{m=1}^{\mc}$, 
    class priors $\Pi_c$ and $\bpi$,
    local step-size $\alpha_l$,
    and local updating iterations $L$.
    \FOR{each client $c\in[C]$}
     \STATE transform $\mathcal{U}_{c}$ to a surrogate labeled dataset $\overline{\mathcal{U}}_{c}$ according to \eqref{surro-set}
     \STATE let $\bg_c=\bQ_c(\boldf)$, where $\bQ_c$ is computed according to Theorem~\ref{theorem1}
    %  \STATE Let $\bg_c=\bQ_c(\boldf)$ and $\mathcal{A}_c$ be a SGD-like optimizer working on $\bg_c$
    \ENDFOR
    \FOR{each round $r = 1, 2,\ldots, R$}
        \STATE broadcast $\fs$ to all the clients $\{\fc\}_{c=1}^C$
        \FOR {each client $c\in[C]$ in parallel}
            \STATE initialize local model $\fc\leftarrow\fs$
            \FOR{$l = 1, 2,\ldots, L$}
                  \STATE fetch mini-batch $\overline{\mathcal{U}}_{mini}$ from $\overline{\mathcal{U}}_{c}$
                  \STATE compute loss $\hat{J}_c(\bg_c;\overline{\mathcal{U}}_{mini})=\frac{1}{n_c}\sum\nolimits_{i=1}^{n_c}\ell(\bQ_c(\boldf(\bx_i)),\overline{y}_i)$
                %   \STATE compute loss $\hat{J}_c(\bg_c;\overline{\mathcal{U}}_{mini})=\frac{1}{n_c}\sum\nolimits_{i=1}^{n_c}\ell(\bg_c(\bx_i),\overline{y}_i)=\frac{1}{n_c}\sum\nolimits_{i=1}^{n_c}\ell(\bQ_c(\boldf(\bx_i)),\overline{y}_i)$
                %   \STATE compute minibatch gradient $\nabla\hat{R}_c(\fc;\overline{\mathcal{U}}_{c})$
                  \STATE $\fc\leftarrow\fc-\alpha_l\cdot\nabla\hat{J}_c(\bg_c;\overline{\mathcal{U}}_{mini})$
            \ENDFOR
        \STATE return $\fc-\fs$ to the server $\fs$
        \ENDFOR
        \STATE $\fs\leftarrow\fs-\alpha_g\cdot\sum\nolimits_{c=1}^C(\fc-\fs)$
    \ENDFOR
    % \STATE \textbf{Output: $\boldf$}
    \end{algorithmic}
\end{algorithm}
\fi
% \Nan{modify the algorithm}


%\iffalse

%\fi

\iffalse
\begin{algorithm}[t]
    \caption{Federation of unsupervised learning~(FedUL)}
    \label{alg}

    \textbf{Server Input:}
    initial $\fs$, 
    global step-size $\alpha_g$,
    and global communication round $R$\\
    \textbf{Client $c$'s Input:}
    local model $\fc$, 
    unlabeled training sets $\mathcal{U}_{c}=\{\mathcal{U}_{c}^{m}\}_{m=1}^{\mc}$, 
    class priors $\Pi_c$ and $\bpi$,
    local step-size $\alpha_l$,
    and local updating iterations $L$
    \begin{algorithmic}[1]
    \State{We start with initializing client data with \textbf{Procedure A}.}
    \State {For $r = 1 \to R$ rounds, we run \textbf{Procedure B} and \textbf{Procedure C} iteratively .}
	\Procedure{\textbf{A}. ClientInit}{$c$} 
     \State transform $\mathcal{U}_{c}$ to a surrogate labeled dataset $\overline{\mathcal{U}}_{c}$ according to \eqref{surro-set}
     \State let $\bg_c=\bQ_c(\boldf)$, where $\bQ_c$ is computed according to Theorem~\ref{theorem1}
    %  \STATE Let $\bg_c=\bQ_c(\boldf)$ and $\mathcal{A}_c$ be a SGD-like optimizer working on $\bg_c$
    \EndProcedure
    
    \Procedure{\textbf{B}. ClientUpdate}{$c$}
    %\State{$\fc\leftarrow\fs$} \Comment{Receive updated model from \textsc{ServerExecute}}
    \State{$\bg_c \leftarrow \bQ_c(\boldf)$} \Comment{Receive updated model from \textsc{ServerExecute} and update surrogate model}
    \For{$l=1\to L$}
                    %   \State{fetch mini-batch $\overline{\mathcal{U}}_{mini}$ from $\overline{\mathcal{U}}_{c}$}
                %   \State { $\hat{J}_c(\bg_c;\overline{\mathcal{U}}_{mini})=\frac{1}{n_c}\sum\nolimits_{i=1}^{n_c}\ell(\bQ_c(\boldf(\bx_i)),\overline{y}_i)$} 
                  \State{ $\bg_c\leftarrow\bg_c-\alpha_l\cdot\nabla\hat{J}_c(\bg_c;\overline{\mathcal{U}}_{c})$}
                  \Comment{SGD updates based on objective \eqref{surro-obj-reformulate}}
    \EndFor
    \State{$\fc\leftarrow \bQ_c^{-1}(\bg_c)$} 
    \Comment{retrieve $\fc$ by dropping the transition layer $\bQ_c$ from $\bg_c$}
                  \State{Send $\fc,\bg_c$ to \textsc{ServerExecute}}
    \EndProcedure{}
    \Procedure{\textbf{C}. ServerExecute}{$r$} 
        \State{Receive local models $\fc,\bg_c$ from \textsc{ClientUpdate}}
        \State{$\fs\leftarrow\fs-\alpha_g\cdot\sum\nolimits_{c=1}^C(\fc-\fs)$}
        \Comment{FL aggregation}
        \State{$\bg\leftarrow\bg-\alpha_g\cdot\sum\nolimits_{c=1}^C(\bg_c-\bg)$}
        \Comment{FL aggregation}
        \State{Broadcast $\fs$ to \textsc{ClientUpdate}}
    \EndProcedure
    \end{algorithmic}
\end{algorithm}
\fi
% \Xiaoxiao{Nan, if you want to rewind your algorithm without error, you need uncomment `usepackage\{algorithmic\}'}

\subsection{Theoretical Analysis}
% With clearly-defined learning objectives, we now proceed to the theoretical analysis on the convergence and optimal model recovery for the proposed method.
In what follows, we provide theoretical analysis on the convergence and optimal model recovery for the proposed method.

\paragraph{Convergence of the Algorithm}
In supervised FL, convergence analysis has been studied with regularity conditions (see Section 3.2.2 in \cite{kairouz2019advances} for a comprehensive survey), e.g.,
the bounded gradient dissimilarity \citep{karimireddy2020scaffold} that associates the client model with the server model for non-IID data distributions.%
\footnote{The IID case is equivalent to batch sampling from the same distribution, where the analysis is less interesting associated with our FL setting and we omit details here.}
In our analysis, we focus on the behaviour of our surrogate learning objective $J$ with the effect from transformation $\bQ_c$. 

\begin{proposition}[Theorem V in \citet{karimireddy2020scaffold}]
\label{prop:convergence}%
Assume that $J(\bg)$ in \eqref{surro-obj} satisfies $\textbf{(A1)}$-$\textbf{(A3)}$ in Appendix~\ref{subsec:prop}.
Denote $\bg^{\ast} = \argmin_{\bg\in\mathcal{G}} \hat{J}(\bg)$, where
$\hat{J}(\bg)=\frac{1}{C}\sum\nolimits_{c=1}^C \hat{J}_c(\bg)\coloneqq\frac{1}{n_c}\sum\nolimits_{i=1}^{n_c}\ell(\bg(\bx_i),\overline{y}_i)$.
Let the global step-size $\alpha_g \geq 1$ and local step-size $\alpha_l \leq \frac{1}{8(1+B^2)\beta L \alpha_g}$,
FedUL given by Algorithm \ref{alg} is expected to have contracting gradient:
with the initialized model $\bg^0$, $F\coloneqq J(\bg^0) - J(\bg^\ast) $ and constant $M=\sigma\sqrt{1+\frac{C}{\alpha_g^2}}$,
in $R$ rounds, the learned model $\bg^R$ satisfies
$$
\E[\| \nabla J(\bg^R)\|^2] \leq \mathcal{O}\left(\frac{\beta M \sqrt{F}}{\sqrt{R L C}} + \frac{\beta^{1/3} (FG)^{2/3}}{{(R+1)^{2/3}}} + \frac{\beta B^2 {F}}{{R}} \right).
$$
% where $M=\sigma\sqrt{1+\frac{C}{\eta_g^2}}$, $D := \|\bg^0 - \bg^{\ast}\| $ and $F :=J(\bg^0) - J(\bg^\ast) $.
% has expected error smaller than $\epsilon$ is upper bounded by
% $
% O_p(\frac{B^2}{\epsilon} + \frac{G}{\epsilon^{3/2}}).
% $
\end{proposition}
Note that the proposition statement is w.r.t. the convergence of $\bg$ learned from the surrogate task.
By model construction, $\bg$ is built from $\bQ_c(\boldf)$.
By Lemma~\ref{lemm:injective}, the convergence of trained model $\bg$ to the optimal model $\bg^{\ast}$ in the function class $\mathcal{G}$ implies the convergence of the retrieved model $\boldf$ to the optimal model $\boldf^{\ast} = \argmin_{\boldf\in\mathcal{F}} \hat{J}(\boldf)$ in the corresponding function class $\mathcal{F}$ (induced by $\mathcal{G}$),
where
% $\hat{J}(\boldf)=\frac{1}{C}\sum\nolimits_{c=1}^C \hat{J}_c(\bQ_c(\boldf))=\frac{1}{n_c}\sum\nolimits_{i=1}^{n_c}\ell(\bQ_c(\boldf(\bx_i)),\overline{y}_i)$.
$\hat{J}(\boldf)=\frac{1}{C}\sum\nolimits_{c=1}^C \hat{J}_c(\bQ_c(\boldf))\coloneqq\frac{1}{n_c}\sum\nolimits_{i=1}^{n_c}\ell(\bQ_c(\boldf(\bx_i)),\overline{y}_i)$ is the empirical version of \eqref{surro-obj-reformulate}.

\paragraph{Optimal Model Recovery}
In our context, the model is optimal in the sense that the minimizer of the surrogate task $J(\boldf;\overline{y})$ 
% in \eqref{surro-obj-reformulate} 
coincide with the minimizer of the supervised task $R(\boldf;y)$ 
% in \eqref{eq:supervised-FL}
, as if all the data have been labeled.
Based on the convergence of surrogate training, we show that FedUL can recover this optimal model.

% \begin{theorem}
% Let $\boldf^{**}=\argmin_\boldf J(\boldf;\overline{y})$ be the optimal classifier learned with \eqref{surro-obj-reformulate},
% and $\boldf^\star=\argmin_\boldf R(\boldf;y)$ be the optimal classifier learned with supervised FL.
% Assume that a proper loss function, e.g., the cross-entropy loss, is chosen for $\ell$, and the model used for learning $\boldf$ is very flexible, e.g., deep neural networks, so that $\boldf^{**}\in\mathcal{F}$.
% % Let $\boldf^{**}$ be the classifier induced by $\bg^{**}$, which is the optimal classifier learned by FedUL, i.e., $\boldf^{**}=\argmin_\boldf J(\boldf;\overline{y})$,
% % and $\boldf^\star=\argmin_\boldf R(\boldf;y)$ be the optimal classifier for supervised FL,
% By assumptions in Proposition~\ref{prop:convergence},
% we have $\boldf^{*}=\boldf^\star$.
% \end{theorem}

% \begin{theorem}
% Let $\bg^{**}=\argmin_\bg J(\bg)$ be the optimal classifier learned with the surrogate learning objective \eqref{surro-obj}.
% Assume that a proper loss function, e.g., the cross-entropy loss, is chosen for $\ell$, and the model used for learning $\bg$ is very flexible, e.g., deep neural networks, so that $\bg^{**}\in\mathcal{G}$.
% Let $\boldf^{**}$ be the classifier induced by $\bg^{**}$, which is the optimal classifier learned by FedUL, i.e., $\boldf^{**}=\argmin_\boldf J(\boldf;\overline{y})$,
% and $\boldf^\star=\argmin_\boldf R(\boldf;y)$ be the optimal classifier for supervised FL,
% by assumptions in Proposition~\ref{prop:convergence},
% we have $\boldf^{**}=\boldf^\star$.
% \end{theorem}

% \begin{theorem}
% \label{thm:optimal}%
% Assume that a proper loss function, e.g., the cross-entropy loss, is chosen for $\ell$, and the model used for $\boldf$ is very flexible, e.g., deep neural networks, so that $\boldf^{**}\in\mathcal{F}$ where $\boldf^{**}=\argmin_\boldf J(\boldf;\overline{y})$.
% Let $\boldf^{\ast} = \argmin_{\boldf\in\mathcal{F}} \hat{J}(\boldf)$ be the optimal classifier learned with FedUL by Algorithm \ref{alg},
% and $\boldf^\star=\argmin_\boldf R(\boldf;y)$ be the optimal classifier learned with supervised FL.
% By assumptions in Proposition~\ref{prop:convergence},
% we have $\boldf^{*}=\boldf^\star$.
% \end{theorem}

\begin{theorem}
\label{thm:optimal}%
Assume that
% a proper loss function, e.g., 
the cross-entropy loss is chosen for $\ell$, and the model used for $\bg$ is very flexible, e.g., deep neural networks, so that $\bg^{**}\in\mathcal{G}$ where $\bg^{**}=\argmin_\bg J(\bg;\overline{y})$.
Let $\boldf^{\ast} = \argmin_{\boldf\in\mathcal{F}} \hat{J}(\boldf)$ be the optimal classifier learned with FedUL by Algorithm \ref{alg},
and $\boldf^\star=\argmin_\boldf R(\boldf;y)$ be the optimal classifier learned with supervised FL.
By assumptions in Proposition~\ref{prop:convergence},
we have $\boldf^{*}=\boldf^\star$.
\end{theorem}





==> Federated Learning with Only Unlabeled Datasets final/sections/proofs.tex <==
\newpage
\section{Proofs}
\label{sec:proof}%

In this appendix, we prove all theorems.

\subsection{Proof of Theorem~\ref{thm:transformation}}
\label{subsec:thm1}%
By the Bayes' rule, $\forall m \in [M]$ we have:
\begin{align}
(\overline{\boldeta}_c(\bx))_m &=
\frac{\overline{p}_c(\bx,\overline{y}=m)}{\overline{p}_c(\bx)}\notag\\
&= \frac{\overline{p}_c(\bx,\overline{y}=m)}{\sum_{m=1}^{\mc}\overline{p}_c(\bx,\overline{y}=m)}\notag\\
&= \frac{\overline{p}_c(\bx\mid\overline{y}=m)\overline{p}_c(\overline{y}=m)}{\sum_{m=1}^{\mc}\overline{p}_c(\bx\mid\overline{y}=m)\overline{p}_c(\overline{y}=m)}\notag\\
&= \frac{p_c^{m}(\bx)\overline{\pi}^m_c}{\sum_{m=1}^{\mc} p_c^{m}(\bx)\overline{\pi}^m_c}\notag\\
&= \frac{\overline{\pi}^m_c\sum\nolimits_{k=1}^K\pi_{c}^{m,k}
p(\bx\mid y=k)}{\sum_{m=1}^{\mc}\overline{\pi}^m_c\sum\nolimits_{k=1}^K\pi_{c}^{m,k}
p(\bx\mid y=k)}\notag\\
&=\frac{\overline{\pi}^m_c\sum\nolimits_{k=1}^K\pi_{c}^{m,k}
\frac{(\boldeta(\bx))_k}{\pi^k}}
{\sum_{m=1}^{\mc}\overline{\pi}^m_c\sum\nolimits_{k=1}^K\pi_{c}^{m,k}
\frac{(\boldeta(\bx))_k}{\pi^k}}.
\label{proof1}
\end{align}
% \overline{\eta}_j(X)&=\frac{\mathbb{P}(X, \overline{Y}=j)}{\overline{\mathbb{P}}(X)}\notag\\
% &=\frac{\mathbb{P}(X\mid \overline{Y}=j)\cdot p(\overline{Y}=j)}{\overline{\mathbb{P}}(X)}\notag\\
% &=\frac{\rho_j\cdot(\sum_{k=1}^K\pi_k^j\mathbb{P}(X\mid Y=k))}
% {\sum^m_{j=1}\rho_j\cdot(\sum_{k=1}^K\pi_k^j\mathbb{P}(X\mid Y=k))}. 
% \label{proof1}
% \end{align}
% On the other hand, by Bayes' rule we have:
% \begin{align}
% \mathbb{P}(X\mid Y=k)&=\frac{\mathbb{P}(Y=k\mid X)\cdot\mathbb{P}(X)}{\mathbb{P}(Y=k)}\notag\\
% &=K\eta_k(X)\mathbb{P}(X)
% \label{proof2}
% \end{align}
% Plug Eq.~\eqref{proof2} into Eq.~\eqref{proof1} we obtain:
% \begin{align}
% \overline{\eta}_j(X)&=
% \frac{\rho_j\cdot(\sum_{k=1}^K\pi_k^j K\eta_k(X)\mathbb{P}(X))}
% {\sum^m_{j=1}\rho_j\cdot(\sum_{k=1}^K\pi_k^j K\eta_k(X)\mathbb{P}(X))}\notag\\
% &=\frac{\rho_j(\sum_{k=1}^K\pi_k^j\eta_k(X))}{\sum_{j=1}^m\rho_j(\sum_{k=1}^K\pi_k^j\eta_k(X))}.
% \label{eta}
% \end{align}
By transforming \eqref{proof1} to the matrix form,
we complete the proof.
\qed

\subsection{Proof of Lemma~\ref{lemm:injective}}
\label{subsec:lemm2}%
Given our data generation process in Section~\ref{sec:formulate}, we have that $\mc\geq k$ and $\Pi_c\in\R^{\mc\times K}$ is a full column rank matrix.
With $D_{\overline{\bpi}_c}$ and $D^{-1}_{\bpi}$ being non-degenerate, we obtain that $\bQ_c(\boldeta(\bx))$ presents an injective mapping from $\boldeta(\bx)$ to $\overline{\boldeta}_c(\bx)$.
\qed

\subsection{Proof of Proposition~\ref{prop:convergence}}
\label{subsec:prop}%
The assumptions $\textbf{(A1)}$-$\textbf{(A3)}$ are listed as follows.
\begin{itemize}
\item[\textbf{(A1)}] Bounded gradient dissimilarity:
    % (G,B)-\textbf{BGD}
    $\exists$ constants $G\geq 0$ and $B \geq 1$ s.t.
\begin{equation*}
    \frac{1}{C}\sum\nolimits_{c=1}^C \|\nabla J_c(\bg) \|^2 \leq G^2 + B^2  \|\nabla J(\bg) \|^2, \forall \bg.
\end{equation*}
\item[\textbf{(A2)}] $\beta$-smooth function $J_c$ satisfies $$\|\nabla J_c(\btheta) - \nabla J_c(\btheta') \| \leq \beta \|\btheta - \btheta'\|, \forall c, \btheta, \btheta'.$$
\item[\textbf{(A3)}] Unbiased stochastic gradient with bounded variance: 
% $\E[\nabla \hat{J}_c(\bg; \overline{\mathcal{U}}_{c})] = \nabla J_c(\bg)$ and
$$\E[\|\nabla \hat{J}_c(\bg; \overline{\mathcal{U}}_{c}) - \nabla J_c(\bg)\|^2] \leq \sigma^2, \forall c, \bg,$$
where $\hat{J}_c(\bg;\overline{\mathcal{U}}_{c})=\frac{1}{n_c}\sum\nolimits_{i=1}^{n_c}\ell(\bg(\bx_i),\overline{y}_i)$.
\end{itemize}
Note that this proposition statement is w.r.t. the convergence of model $\bg$ learned from the surrogate supervised learning task.
The proof follows directly from Theorem V in \citet{karimireddy2020scaffold}.
\qed

\subsection{Proof of Theorem~\ref{thm:optimal}}
\label{subsec:opt}%
When a proper loss \citep{reid2010composite} is used for $\ell$, the mapping of $\bg^{**}$ is the unique minimizer of $J(\bg)$.
We show an example of the a widely used proper loss function: the cross-entropy loss \citep{de2005tutorial} defined as
$$\ell_{\rm{ce}}(\bg(\bx),\overline{y})=-\sum\nolimits_{m=1}^M\boldsymbol{1}(\overline{y}=m)\log(\bg(\bx))_{m}=-\log(\bg(\bx))_{\overline{y}}.$$

We can see that the cross-entropy loss is non-negative by its definition.
Therefore, minimizing $J(\bg)$ can be obtained by minimizing the conditional risk $\mathbb{E}_{p(\overline{y}\mid \boldsymbol{x})}[\ell(\bg(\bx),\overline{y})\mid \boldsymbol{x}]$ for every $\boldsymbol{x} \in \mathcal{X}$. So we are now optimizing
        \begin{equation} \nonumber
            \begin{gathered}
             \phi(\bg)=-\sum_{m=1}^{M}p(\overline{y}=m\mid \boldsymbol{x})\cdot \log(g(\boldsymbol{x}))_m, \quad {\rm{s.t.}} \sum_{m=1}^{M} (g(\boldsymbol{x}))_m=1.
            \end{gathered}
        \end{equation}
        By using the Lagrange multiplier method \citep{bertsekas1997nonlinear}, we have
        \begin{equation} \nonumber
            \mathcal{L}=-\sum_{m=1}^{M}p(\overline{y}=m\mid \boldsymbol{x})\cdot \log(g(\boldsymbol{x}))_m-\lambda\cdot(\sum_{m=1}^{M}(g(\boldsymbol{x}))_m-1).
        \end{equation}
        The derivative of $\mathcal{L}$ with respect to $\boldsymbol{g}$ is
        \begin{equation} \nonumber
            \frac{\partial\mathcal{L}}{\partial\boldsymbol{g}} = \left[-\frac{p(\overline{y}=1\mid \boldsymbol{x})}{(\bg(\boldsymbol{x}))_1}-\lambda,\cdot\cdot\cdot,-\frac{p(\overline{y}=M\mid \boldsymbol{x})}{(\bg(\boldsymbol{x}))_M}-\lambda\right]^{\top}.
        \end{equation}
        By setting this derivative to 0 we obtain
        \begin{equation} \nonumber
            (\bg(\boldsymbol{x}))_m=-\frac{1}{\lambda}\cdot p(\overline{y}=m\mid \boldsymbol{x}), \quad \forall m=1,\ldots,M \ \ {\rm{and}}\ \  \forall \boldsymbol{x} \in \mathcal{X}.    
        \end{equation}
        Since $\boldsymbol{g} \in \Delta_{M-1}$ is the $M$-dimensional simplex, we have $\sum_{m=1}^{M}(\bg^{**}(\boldsymbol{x}))_m=1$ and $\sum_{m=1}^{M}p(\overline{y}=j\mid \boldsymbol{x})=1$.
        Then
        \begin{equation} \nonumber
            \sum_{m=1}^{M}(\bg^{**}(\boldsymbol{x}))_m=-\frac{1}{\lambda}\cdot\sum_{m=1}^{M}p(\overline{y}=m\mid \boldsymbol{x})=1.
        \end{equation}
        Therefore we obtain $\lambda=-1$ and $(\bg^{**}(\boldsymbol{x}))_m=p(\overline{y}=m\mid \boldsymbol{x})=(\overline{\eta}(\boldsymbol{x}))_m,\forall m = 1,\ldots,M$ and $\forall \boldsymbol{x} \in \mathcal{X}$, which is equivalent to $\boldsymbol{g}^{**}(\bx) = \bar{\boldsymbol{\eta}}(\bx)$. Similarly, we obtain \begin{align}
        \label{optimal1}
        \boldf^\star(\bx)=\boldeta(\bx).
        \end{align}
Given Proposition~\ref{prop:convergence} and the assumption that the model used for $\bg$ is sufficiently flexible,
we obtain that the classification model learned by FedUL (see Algorithm \ref{alg}) satisfies $\bg^{\ast}=\bg^{**}$.
By our model construction, $\bg$ is built from $\bQ_c(\boldf)$.
Then we have 
\begin{align}
\label{optimal2}
\boldf^{\ast}=\boldf^{**}
\end{align}
% $\boldf^{\ast}=\boldf^{**}$ 
where $\boldf^{**}=\argmin_\boldf J(\boldf)$ is the model induced by $\bg^{**}$.
Given Theorem~\ref{thm:transformation} and Lemma~\ref{lemm:injective},
we obtain that $\boldsymbol{g}^{**}(\bx) = \bar{\boldsymbol{\eta}}(\bx)$ if and only if 
\begin{align}
\label{optimal3}
\boldf^{**}(\bx)={\boldsymbol{\eta}}(\bx).
\end{align}
% $\boldf^{**}(\bx)={\boldsymbol{\eta}}(\bx)$.
By summarizing \eqref{optimal1}, \eqref{optimal2}, and \eqref{optimal3} we obtain $\boldf^{*}=\boldf^\star$.
\qed

==> Federated Learning with Only Unlabeled Datasets final/sections/statement.tex <==
\section*{Ethics Statement}
Collecting sample-wise labels for training can be costly and may violate data privacy. Considering data in the real world are often distributed at a large scale,
% collected distributed, 
we provide a promising solution to perform multi-class classification on distributed U data in the FL system. Our method FedUL can be widely applied to data-sensitive fields, such as healthcare, politics, and finance, where the sample-wise label is not available, but populational prevalence can be accessed.  With FedUL, we hope the future FL can enjoy significant labeling cost reduction and improve its privacy. 
% Therefore, we believe our proposed method and its potential application have a positive impact on society.
The real datasets used in this work are publicly available with appropriate prepossessing to de-identify patients' identities. We provide proper references to the datasets, libraries, and tools used in our study. This study does not have any legal compliance, conflict of interest, or research integrity issues. 

\section*{Reproducibility Statement}
We provide the codes to reproduce the main experimental results at \url{https://github.com/lunanbit/FedUL}.
% via the  \href{https://drive.google.com/drive/folders/1kcMO0_XoxoPFhv1ZgcZ6bV_HTzZo-zPs?usp=sharing}{anonymous download link} indicated in Appendix. 
We further provide experimental details and additional information of the datasets in the supplementary materials.

==> Federated Learning with Only Unlabeled Datasets final/theory.tex <==
% \newpage
\section{Theoretical Analyses}
\label{sec:theory}
In this section, we theoretically show the convergence of FedUL and prove that the optimal FL model can be identified even without any labeled data.

% \subsection{Problem Formulation}
% \label{sec:formulation}
\paragraph{Convergence of the algorithm}

\paragraph{Optimal model recovery}

% \paragraph{Notation}
% We let the $t$-th global rounds, server broadcast global weights $u(t) \in \R^{d \times m}$ to every client. Each client $c$ then start from local weights $w_{0,c}(t) = u(t)$ and do $K$ (local) steps gradient descent to find $w_{K,c}(t)$.  Each client send $\Delta u_c(t) = w_{K,c}(t)-w_{0,c}(t)$ to server. Server compute a new $u(t+1)$ based on the average of all $\Delta u_c(t)$. Specifically, the server update $u(t)$ by the average of all local update $\Delta u_c(t)$ and arrive at $u(t+1) = u(t) + \eta_\glo \cdot \sum_{c \in [N]} \Delta u_c(t) /N$.

% \paragraph{Setup}

% We define one-hidden layer neural network function $f : \R^d \rightarrow \R$ similar as \cite{dzps19,sy19}
% \begin{align*}
%     f (u,x) := \frac{1}{ \sqrt{m} } \sum_{r=1}^m a_r \phi ( u_r^\top x ),
% \end{align*}
%  where $u \in \R^{d \times m}$ and $u_r \in \R^d$ is the $r$-th column of matrix $u$.
% \begin{definition}[Initialization]\label{def:initialization}
% We initialize $u \in \R^{d \times m}$ and $a \in \R^m$ as follows:
% \begin{itemize}
%     \item For each $r$, $u_r$ is sampled from ${\cal N}(0,\sigma^2 I)$ 
%     \item For each $r$, $a_r$ is sampled from $\{-1,+1\}$ uniformly at random (we don't need to train).
% \end{itemize}
% \end{definition}
% %where $a \in \{-1,+1\}^m$ (we don't need to train), and $u \in \R^{d \times m}$ where $u_r \in \R^d$ is the $r$-th column of matrix $u$.

% We define the Loss function for $j \in [N]$,
% \begin{align*}
%     L_j (u,x): = & ~ \frac{1}{2} \sum_{i \in S_j} ( f(u,x_i) - y_i )^2, \\
%     L(u,x) := & ~ \frac{1}{N} \sum_{j=1}^N  L_j(u,x).
% \end{align*}

% We can compute the gradient $\frac{ \partial f(u,x)}{ \partial u_r } \in \R^d$ (of function $f$),
% \begin{align*}
%     \frac{ \partial f(u,x)}{ \partial u_r } = \frac{1}{ \sqrt{m} } a_r x {\bf 1}_{ u_r^\top x \geq 0 } .
% \end{align*}

% We can compute the gradient $ \frac{ \partial L_c (u) }{ \partial u_r } \in \R^d $ (of function $L$),
% \begin{align*}
%     \frac{ \partial L_c (u) }{ \partial u_r } = \frac{1}{\sqrt{m}} \sum_{i = 1}^n ( f(u,x_i) - y_i) a_r x_i {\bf 1}_{ u_{r,c}^\top x_i \geq 0 } .
% \end{align*}

% We formalize the problem as minimizing the sum of loss functions over all clients:
% \begin{align*}
%     \min _{u \in \mathbb{R}^{d \times M}}
%     L(u).
% \end{align*}

% \paragraph{Local update}

% In each local step, we update $w_{k,c}$ by gradient descent.

% \begin{align*}
%     w_{k+1,c} \leftarrow w_{k,c} -  \eta_{\loc}\cdot \frac{ \partial L_c (w_{k,c}) }{ \partial w_{k,c} }.
% \end{align*}
% Note that 
% \begin{align*}
%      \frac{ \partial L_c (w_{k,c}) }{ \partial w_{k,c,r} }=  \frac{1}{\sqrt{m}} \sum_{i \in S_c} ( f(w_{k,c},x_i) - y_i) a_r x_i {\bf 1}_{ w_{k,c,r}^\top x_i \geq 0 }.
% \end{align*}

% \paragraph{Global aggregation}

% In each global communication round we aggregate all local updates of clients by taking a simple average
% \begin{align*}
%     \Delta u(t) = \sum_{c \in [N]}\Delta u_c(t) / N ,
% \end{align*}
% where $\Delta u_c(t) = w_{K,c} - w_{0,c}$ for all $c \in [N]$.

% \paragraph{Global steps in total}

% Then global model simply add $\Delta u(t)$ to its parameters.
% \begin{align*}
%     u(t+1) \leftarrow u(t) + \eta_{\glo} \cdot \Delta u(t).
% \end{align*}
% \subsection{Convergence}
% \label{sec:convergence}

% The main theoretical result of this work, the convergence result of federated learning in neural networks, is presented in the following theorem.
% \begin{theorem}[Convergence of FedAvg, \cite{hlsy21}]\label{thm:main_informal}
% Let $m = \Omega( \lambda^{-4} n^4 \log (n/\delta) )$, we i.i.d. initialize $u_r(0)$, $a_r$ as Definition~\ref{def:initialization} where $\sigma = 1$. Let $\lambda$ denote $\lambda_{\min}(H(0))$. Let $\kappa$ denote the condition number of $H(0)$ 
% . For $N$ clients, for any $\epsilon$, let
% \begin{align*}
% T=O \Big( \frac{N}{\lambda\eta_{\loc}\eta_{\glo}K}\cdot \log(1/\epsilon) \Big)
% \end{align*}
% there is an algorithm (FL-NTK) runs in $T$ global steps and each client runs $K$ local steps with choosing 
% \begin{align*}
%     \eta_{\loc} = O\Big( \frac{\lambda}{\kappa Kn^2} \Big) \mathrm{~~~and~~~} \eta_{\glo} = O(1)
% \end{align*} 
% and outputs weight $U$ with probability at least $1-\delta$ such that the training loss $L(u,x)$ satisfies
% \begin{align*}
%     L(u,x)=\frac{1}{2N}\sum_{i=1}^N(f(u,x_i)-y_i)^2 \leq \epsilon .
% \end{align*}
% \end{theorem}

% To show an upper bound for the generalization error of federated learning in neural networks, we make additional assumptions on the training data distribution $\mathcal{D}_{\rm tr}$ and test data distribution $\mathcal{D}_{\rm te}$ following \cite{adh+19a,sy19,hlsy21}.

% \begin{definition}[Non-degenerate Data Distribution, Definition 5.1 in \cite{adh+19a}]
% A distribution $\mathcal{D}$ over $\mathbb{R}^d\times\mathbb{R}$ is \emph{$(\lambda,\delta,n)$-non-degenerate},
% if with probability at least $1-\delta$,
% for $n$ i.i.d samples $(x_i,y_i)_{i=1}^n$ chosen from $\mathcal{D}$,
% $\lambda_{\min}(H(0))\geq \lambda>0$.
% \end{definition}

% \begin{theorem}[Generalization bound of FedAvg, \cite{hlsy21}]
% \label{thm:generalization_main_informal}
% Fix failure probability $\delta \in (0,1)$.
% Suppose the training data $S=\{(x_i,y_i)\}_{i=1}^n$ are i.i.d samples from a $(\lambda,\delta/3,n)$-non-degenerate distribution $\mathcal{D}$,
% and 
% \begin{itemize} 
% \item $\sigma\leq O({\lambda \cdot \poly(\log n,\log(1/\delta))}/{n})$,
% \item 
% $m\geq \Omega ( \sigma^{-2} \cdot \poly(n,\log m,\log(1/\delta),\lambda^{-1}) )$,
% \item $T\geq \Omega ( ( \eta_{\loc}\eta_{\glo}K\lambda )^{-1} N \log(n/\delta) )$ .
% \end{itemize}
% We initialize $u \in \R^{d \times m }$ and $a \in \R^m$ as Definition~\ref{def:initialization}. 
% Consider any loss function $\ell:\mathbb{R}\times \mathbb{R}\rightarrow [0,1]$ that is 1-Lipschitz in its first argument.
% Then with probability at least $1-\delta$ the following event happens: after $T$  global steps,  the generalization loss 
% \begin{align*}
%     L_{\mathcal{D}}(f)=\E_{(x,y)\sim \mathcal{D}}[\ell(f(u,x),y)]
% \end{align*}
% is upper bounded as
% \begin{align*}
% L_{\mathcal{D}}(f)\leq & ~ ( {2y^\top (H^{\infty})^{-1}y}/{n} )^{1/2} +O (\sqrt{ \log(n / (\lambda \delta) ) / n} ).
% \end{align*}
% \end{theorem}
% \iffalse
% \begin{remark}
% We would like to comment two insights drawn from the above theorem concerning the number of iteration in federated learning. First, more number of iteration is required with more clients. This is intuitive in federated learning since the data in different clients are usually not identically distributed, causing additional communication rounds for the model to learn. Secondly, the number of local steps reduces the number of iteration when local learning rate is sufficiently small. This happens when local models are more effective in learning from local data. However, clients may over-fit to local data as the number of local steps increases, which jeopardizes the federated learning as a whole. This is conceptually shown in the intricacy of the choice of local learning rates.
% \end{remark}
% \fi




==> cmds.tex <==
\makeatletter
% Taken from http://ctan.org/pkg/centernot
\newcommand*{\centernot}{%
  \mathpalette\@centernot
}
\def\@centernot#1#2{%
  \mathrel{%
    \rlap{%
      \settowidth\dimen@{$\m@th#1{#2}$}%
      \kern.5\dimen@
      \settowidth\dimen@{$\m@th#1=$}%
      \kern-.5\dimen@
      $\m@th#1\not$%
    }%
    {#2}%
  }%
}
\makeatother
\newcommand{\independent}{\perp\mkern-9.5mu\perp}
\newcommand{\dependent}{\centernot{\independent}}



% \newtheorem{theorem}{Theorem}[section]
\newtheorem{rul}[theorem]{Rule}

==> related.tex <==
\section{Related Works}

To the best of our knowledge, this is the first work addressing the FL with only unlabeled datasets

\paragraph{Federated learning}
Federated learning is an emerging paradigm in distributed machine learning, which allows different clients collaboratively train model together without data sharing. One of the most popular FL paradigm is called FedAvg~\cite{mcmahan2017communication}. FedAvg is a easy-to-implement distributed learning strategy by aggregating local model updates on the server side and transmitting the averaged model back to local clients. For IID data, FL has been proven effective. However, in practice, data mostly distribute as non-IID. Non-IID data could substantially degrade the performance of FL models~\cite{zhao2018federated,li2019convergence, li2021fedbn}. Several approaches have been proposed to address the non-IID issue. FedProx \citep{li2018federated}, a recent provable framework tackled the heterogeneity by adding a proximal term to FedAvg to regularize local model weights updates. Scaffold~\cite{karimireddy2020scaffold} corrects the local updates by variance reduction. FedRobust \citep{reisizadeh2020robust} assumes data follows an affine distribution shift and tackles this problem by learning the affine transformation. FedBN~\cite{li2021fedbn} keeps all BN parameters strictly local to reduce the effect of feature shift. However, almost all of theses existing FL studies demonstrate that their approaches are better than FedAvg on  non-IID data in supervised learning only. It is still an open question whether FedAvg is a feasible strategy for unlabeled data leanring. 

% Add Personalized non-IID

% Add Weakly Supervsied FL



%Introduce standard FedAvg, non i.i.d.

\paragraph{Unlabeled data learning}

\begin{itemize}
    \item Federated Learning with Only Positive Labels (ICML2020) \url{http://www.sanjivk.com/FedPositive_ICML20.pdf};
    \item Federated Semi-Supervised Learning with Inter-Client Consistency and Disjoint Learning (ICLR2021) \url{https://arxiv.org/pdf/2006.12097.pdf}
    \item FEDAUX: Leveraging Unlabeled Auxiliary Data in Federated Learning (arxiv) \url{https://arxiv.org/pdf/2102.02514.pdf};
    \item Federated Learning with Positive and Unlabeled Data (arxiv) \url{https://arxiv.org/pdf/2106.10904v1.pdf};
    \item SemiFL: Communication Efficient Semi-Supervised Federated Learning with Unlabeled Clients (arxiv) \url{https://arxiv.org/pdf/2106.01432.pdf}.
    \item Learning from Corrupted Binary Labels via Class-Probability Estimation, ICML2015,
    \url{http://proceedings.mlr.press/v37/menon15.pdf}
    \item Learning from Label Proportions with Generative Adversarial Networks, NIPS2019
    \url{https://arxiv.org/abs/1909.02180}
    \item On the minimal supervision for training any binary classifier from only unlabeled data, ICLR2019, 
    \url{https://arxiv.org/abs/1808.10585}
    \item Mitigating overfitting in supervised classification from two unlabeled datasets: A consistent risk correction approach, AISTATS2020, \url{https://arxiv.org/abs/1910.08974}
    \item Learning from label proportions: A mutual contamination framework, NIPS2020, \url{https://arxiv.org/abs/2006.07330}
    \item Learning from label proportions with consistency regularization, ACML2020,  \url{https://www.csie.ntu.edu.tw/~htlin/paper/doc/acml20llpvat.pdf}
\end{itemize}




==> theory.tex <==
% \newpage
\section{Theoretical Analyses}
\label{sec:theory}
In this section, we theoretically show the convergence of FedUL and prove that the optimal FL model can be identified even without any labeled data.

% \subsection{Problem Formulation}
% \label{sec:formulation}
\paragraph{Convergence of the algorithm}

\paragraph{Optimal model recovery}

% \paragraph{Notation}
% We let the $t$-th global rounds, server broadcast global weights $u(t) \in \R^{d \times m}$ to every client. Each client $c$ then start from local weights $w_{0,c}(t) = u(t)$ and do $K$ (local) steps gradient descent to find $w_{K,c}(t)$.  Each client send $\Delta u_c(t) = w_{K,c}(t)-w_{0,c}(t)$ to server. Server compute a new $u(t+1)$ based on the average of all $\Delta u_c(t)$. Specifically, the server update $u(t)$ by the average of all local update $\Delta u_c(t)$ and arrive at $u(t+1) = u(t) + \eta_\glo \cdot \sum_{c \in [N]} \Delta u_c(t) /N$.

% \paragraph{Setup}

% We define one-hidden layer neural network function $f : \R^d \rightarrow \R$ similar as \cite{dzps19,sy19}
% \begin{align*}
%     f (u,x) := \frac{1}{ \sqrt{m} } \sum_{r=1}^m a_r \phi ( u_r^\top x ),
% \end{align*}
%  where $u \in \R^{d \times m}$ and $u_r \in \R^d$ is the $r$-th column of matrix $u$.
% \begin{definition}[Initialization]\label{def:initialization}
% We initialize $u \in \R^{d \times m}$ and $a \in \R^m$ as follows:
% \begin{itemize}
%     \item For each $r$, $u_r$ is sampled from ${\cal N}(0,\sigma^2 I)$ 
%     \item For each $r$, $a_r$ is sampled from $\{-1,+1\}$ uniformly at random (we don't need to train).
% \end{itemize}
% \end{definition}
% %where $a \in \{-1,+1\}^m$ (we don't need to train), and $u \in \R^{d \times m}$ where $u_r \in \R^d$ is the $r$-th column of matrix $u$.

% We define the Loss function for $j \in [N]$,
% \begin{align*}
%     L_j (u,x): = & ~ \frac{1}{2} \sum_{i \in S_j} ( f(u,x_i) - y_i )^2, \\
%     L(u,x) := & ~ \frac{1}{N} \sum_{j=1}^N  L_j(u,x).
% \end{align*}

% We can compute the gradient $\frac{ \partial f(u,x)}{ \partial u_r } \in \R^d$ (of function $f$),
% \begin{align*}
%     \frac{ \partial f(u,x)}{ \partial u_r } = \frac{1}{ \sqrt{m} } a_r x {\bf 1}_{ u_r^\top x \geq 0 } .
% \end{align*}

% We can compute the gradient $ \frac{ \partial L_c (u) }{ \partial u_r } \in \R^d $ (of function $L$),
% \begin{align*}
%     \frac{ \partial L_c (u) }{ \partial u_r } = \frac{1}{\sqrt{m}} \sum_{i = 1}^n ( f(u,x_i) - y_i) a_r x_i {\bf 1}_{ u_{r,c}^\top x_i \geq 0 } .
% \end{align*}

% We formalize the problem as minimizing the sum of loss functions over all clients:
% \begin{align*}
%     \min _{u \in \mathbb{R}^{d \times M}}
%     L(u).
% \end{align*}

% \paragraph{Local update}

% In each local step, we update $w_{k,c}$ by gradient descent.

% \begin{align*}
%     w_{k+1,c} \leftarrow w_{k,c} -  \eta_{\loc}\cdot \frac{ \partial L_c (w_{k,c}) }{ \partial w_{k,c} }.
% \end{align*}
% Note that 
% \begin{align*}
%      \frac{ \partial L_c (w_{k,c}) }{ \partial w_{k,c,r} }=  \frac{1}{\sqrt{m}} \sum_{i \in S_c} ( f(w_{k,c},x_i) - y_i) a_r x_i {\bf 1}_{ w_{k,c,r}^\top x_i \geq 0 }.
% \end{align*}

% \paragraph{Global aggregation}

% In each global communication round we aggregate all local updates of clients by taking a simple average
% \begin{align*}
%     \Delta u(t) = \sum_{c \in [N]}\Delta u_c(t) / N ,
% \end{align*}
% where $\Delta u_c(t) = w_{K,c} - w_{0,c}$ for all $c \in [N]$.

% \paragraph{Global steps in total}

% Then global model simply add $\Delta u(t)$ to its parameters.
% \begin{align*}
%     u(t+1) \leftarrow u(t) + \eta_{\glo} \cdot \Delta u(t).
% \end{align*}
% \subsection{Convergence}
% \label{sec:convergence}

% The main theoretical result of this work, the convergence result of federated learning in neural networks, is presented in the following theorem.
% \begin{theorem}[Convergence of FedAvg, \cite{hlsy21}]\label{thm:main_informal}
% Let $m = \Omega( \lambda^{-4} n^4 \log (n/\delta) )$, we i.i.d. initialize $u_r(0)$, $a_r$ as Definition~\ref{def:initialization} where $\sigma = 1$. Let $\lambda$ denote $\lambda_{\min}(H(0))$. Let $\kappa$ denote the condition number of $H(0)$ 
% . For $N$ clients, for any $\epsilon$, let
% \begin{align*}
% T=O \Big( \frac{N}{\lambda\eta_{\loc}\eta_{\glo}K}\cdot \log(1/\epsilon) \Big)
% \end{align*}
% there is an algorithm (FL-NTK) runs in $T$ global steps and each client runs $K$ local steps with choosing 
% \begin{align*}
%     \eta_{\loc} = O\Big( \frac{\lambda}{\kappa Kn^2} \Big) \mathrm{~~~and~~~} \eta_{\glo} = O(1)
% \end{align*} 
% and outputs weight $U$ with probability at least $1-\delta$ such that the training loss $L(u,x)$ satisfies
% \begin{align*}
%     L(u,x)=\frac{1}{2N}\sum_{i=1}^N(f(u,x_i)-y_i)^2 \leq \epsilon .
% \end{align*}
% \end{theorem}

% To show an upper bound for the generalization error of federated learning in neural networks, we make additional assumptions on the training data distribution $\mathcal{D}_{\rm tr}$ and test data distribution $\mathcal{D}_{\rm te}$ following \cite{adh+19a,sy19,hlsy21}.

% \begin{definition}[Non-degenerate Data Distribution, Definition 5.1 in \cite{adh+19a}]
% A distribution $\mathcal{D}$ over $\mathbb{R}^d\times\mathbb{R}$ is \emph{$(\lambda,\delta,n)$-non-degenerate},
% if with probability at least $1-\delta$,
% for $n$ i.i.d samples $(x_i,y_i)_{i=1}^n$ chosen from $\mathcal{D}$,
% $\lambda_{\min}(H(0))\geq \lambda>0$.
% \end{definition}

% \begin{theorem}[Generalization bound of FedAvg, \cite{hlsy21}]
% \label{thm:generalization_main_informal}
% Fix failure probability $\delta \in (0,1)$.
% Suppose the training data $S=\{(x_i,y_i)\}_{i=1}^n$ are i.i.d samples from a $(\lambda,\delta/3,n)$-non-degenerate distribution $\mathcal{D}$,
% and 
% \begin{itemize} 
% \item $\sigma\leq O({\lambda \cdot \poly(\log n,\log(1/\delta))}/{n})$,
% \item 
% $m\geq \Omega ( \sigma^{-2} \cdot \poly(n,\log m,\log(1/\delta),\lambda^{-1}) )$,
% \item $T\geq \Omega ( ( \eta_{\loc}\eta_{\glo}K\lambda )^{-1} N \log(n/\delta) )$ .
% \end{itemize}
% We initialize $u \in \R^{d \times m }$ and $a \in \R^m$ as Definition~\ref{def:initialization}. 
% Consider any loss function $\ell:\mathbb{R}\times \mathbb{R}\rightarrow [0,1]$ that is 1-Lipschitz in its first argument.
% Then with probability at least $1-\delta$ the following event happens: after $T$  global steps,  the generalization loss 
% \begin{align*}
%     L_{\mathcal{D}}(f)=\E_{(x,y)\sim \mathcal{D}}[\ell(f(u,x),y)]
% \end{align*}
% is upper bounded as
% \begin{align*}
% L_{\mathcal{D}}(f)\leq & ~ ( {2y^\top (H^{\infty})^{-1}y}/{n} )^{1/2} +O (\sqrt{ \log(n / (\lambda \delta) ) / n} ).
% \end{align*}
% \end{theorem}
% \iffalse
% \begin{remark}
% We would like to comment two insights drawn from the above theorem concerning the number of iteration in federated learning. First, more number of iteration is required with more clients. This is intuitive in federated learning since the data in different clients are usually not identically distributed, causing additional communication rounds for the model to learn. Secondly, the number of local steps reduces the number of iteration when local learning rate is sufficiently small. This happens when local models are more effective in learning from local data. However, clients may over-fit to local data as the number of local steps increases, which jeopardizes the federated learning as a whole. This is conceptually shown in the intricacy of the choice of local learning rates.
% \end{remark}
% \fi



